An Upper Bound on the M/M/k Queue With Deterministic Setup Times

In many systems, servers do not turn on instantly; instead, a setup time must pass before a server can begin work. These "setup times" can wreak havoc on a system's queueing; this is especially true in modern systems, where servers are regularly turned on and off as a way to reduce operating costs (energy, labor, CO2, etc.). To design modern systems which are both efficient and performant, we need to understand how setup times affect queues. Unfortunately, despite successes in understanding setup in a single-server system, setup in a multiserver system remains poorly understood. To circumvent the main difficulty in analyzing multiserver setup, all existing results assume that setup times are memoryless, i.e. distributed Exponentially. However, in most practical settings, setup times are close to Deterministic, and the widely used Exponential-setup assumption leads to unrealistic model behavior and a dramatic underestimation of the true harm caused by setup times. This paper provides a comprehensive characterization of the average waiting time in a multiserver system with Deterministic setup times, the M/M/k/Setup-Deterministic. In particular, we derive upper and lower bounds on the average waiting time in this system, and show these bounds are within a multiplicative constant of each other. These bounds are the first closed-form characterization of waiting time in any finite-server system with setup times. Further, we demonstrate how to combine our upper and lower bounds to derive a simple and accurate approximation for the average waiting time. These results are all made possible via a new technique for analyzing random time integrals that we named the Method of Intervening Stopping Times, or MIST.

==> 4_results__.tex <==
\paragraph{Summary.} We now state our three main results concerning the average queue length $\ex{Q(\infty)}$: an approximation, an upper bound, and a lower bound. 
Note that, by Little's Law \citep{Kle_75}, which states that $\ex{Q(\infty)} = k\lambda \ex{T_Q}$, our results immediately translate to results on the average waiting time $\ex{T_Q}$; see Figure~\ref{fig:boundComparison} for an illustration. 
Our first main result, Approximation~\ref{apx:only}, is a simple and accurate approximation to the average queue length $\ex{Q(\infty)}$; we demonstrate its accuracy in Figure~\ref{fig:approxEval}.
Our second main result, the upper bound of Theorem~\ref{thm:main}, is the first-ever upper bound on the average queue length $\ex{Q(\infty)}$ in a multiserver system with Deterministic setup times. 
By contrast, our third main result, the lower bound of Theorem~\ref{thm:improvement}, is only the second lower bound on the queue length $\ex{Q(\infty)}$; however, improving on the lower bound of \citep{WHW}, we show that our bounds differ by at most a multiplicative constant. 
Notably, all three results are in explicit closed-form, unlikely nearly all other results concerning multiserver systems with setup times.

\chmade{
We begin by discussing Approximation~\ref{apx:only} in Section~\ref{sec:apx_statement}.
We then state the exact forms of the upper and lower bounds in Theorems~\ref{thm:main} and~\ref{thm:improvement} in Sections~\ref{sec:upper-statement} and \ref{sec:lower-statement}, respectively, whose proofs are given in Sections~\ref{sec:proof} and~\ref{sec:improvement}, respectively.
We then discuss the order of these bounds in Section~\ref{sec:discussion_of_bnds}.
}

\subsection{Approximation: Statement and Evaluation}\label{sec:apx_statement}

\begin{restatable}[Approximation of the Average Queue Length]{apprx}{ourapx}\label{apx:only}
    Let $\capx \triangleq \sqrt{\frac{\pi}{2}}$. Then, if the offered load $R\triangleq k \rho > 1$, one can approximate the steady state queue length as
    \begin{equation}\label{eq:full}
        \ex{Q(\infty)} \approx Q_{\textup{apx}} \triangleq 
        \frac{
            \frac{1}{2} \mu \beta^2 \capx \sqrt{R} + 
            \frac{\mu \beta \capx \sqrt{R}} {\mu k(1-\rho)}
            \left[
                \frac{\mu \beta \capx \sqrt{R} + 1}{2} + \frac{1}{1-\rho}
            \right]
        }
        {
            \beta + \frac{\mu \beta \capx \sqrt{R} }{\mu k (1-\rho)}
        }.
    \end{equation}

        On the other hand, if $R < 1$, then a better approximation is
    \begin{equation}\label{eq:single-serv-approx}
        \ex{Q\left(\infty\right)} \approx \frac{\mu R \beta}{2}\left[\frac{2 + \mu R \beta}{1 + \mu R \beta}\right].
    \end{equation}
\end{restatable}

\begin{figure}
    \centering
    \includegraphics[ trim={1cm 1cm 0 0},clip, width=0.9\textwidth]{figures/multi_sweep_ss_inc.pdf}
    \caption{Simulation results demonstrating the high accuracy of Approximation~\ref{apx:only}. For each of these 9 plots, we plot the behavior of the average waiting time as one varies the load $\rho$ from $0$ to $1$, holding fixed the total number of servers $k$ as well as the setup time $\beta$. In each row, we hold the number of servers $k$ constant while testing increasing values of the setup times $\beta$. In each column, we hold the setup time $\beta$ constant while increasing the number of servers. We plot three quantities: 1) in black, the simulated average waiting time for the M/M/k/Setup-Deterministic; 2)in purple, the predicted average waiting time of Approximation~\ref{apx:only}; and \chmade{3) the predicted average waiting time of as given by the ``low-R'' approximation of \eqref{eq:ss_approx}, a variation on the single-server setup result of \cite{welchfirstservice}.  We also include, as a reference, a dotted line illustrating the point at which the offered load $R\triangleq k\rho = 1$. Our approximation works well when the average number of busy servers $R > 1$, and the ``low-R'' approximation works well when $R < 1$.}}
\label{fig:approxEval}
\end{figure}

\paragraph{Evaluation.} 
%Our third and final result is Approximation~\ref{apx:only}.
Approximation~\ref{apx:only} represents a significant expansion of our understanding of the M/M/$k$/Setup-Deterministic.
From a practical standpoint, we observe in Figure~\ref{fig:approxEval} that our approximation is extremely accurate across a wide range of system parameters.
Moreover, the formula itself is simple enough that one can use it to rapidly answer provisioning questions.

Approximation~\ref{apx:only} is also interesting from a theoretical perspective.
It 


In Figure~\ref{fig:approxEval}, we observe that our approximation is accurate across a wide range of system parameters, so long as the offered load $R > 1$, a considerable weakening of the assumptions used in our proofs.
In that sense, it serves as a testament to the strength of our approach that our resulting approximation remains accurate all the way down to offered loads $R < 1$.
And, while offered loads $R < 1$ are of limited practical interest, when the offered load is that small, we anticipate that the waiting time exhibits a ``single-server bottleneck'' effect, mirroring the behavior in \citep{welchfirstservice}. 
\chmade{
In particular, in the M/M/1/Setup-Deterministic, one finds in \citep{welchfirstservice} that
\begin{equation*}
    \ex{T_Q} = \frac{1}{\mu - \lambda} + \frac{\beta}{2}\left[\frac{2 + \lambda \beta}{1 + \lambda \beta}\right].
\end{equation*}
Taking the second term, which measures the additional wait in the system due to setup times, and using $R$ in place of $\frac{\lambda}{\mu}$, we obtain a ``low-$R$'' approximation
\begin{equation}\label{eq:ss_approx}
    \ex{T_Q} \approx \frac{\beta}{2}\left[\frac{2 + \mu R \beta}{1 + \mu R \beta}\right].
\end{equation}
We include this ``low-R'' approximation in Figure~\ref{fig:approxEval} and note that, when $R < 1$, this approximation seems to capture the performance behavior very well.}


\paragraph{Assumptions.} In our theorems, in order to more simply characterize the system's behavior, we make two assumptions.
First, we assume that setup times are large compared to service time, i.e. the average setup time $\beta \geq 100\frac{1}{\mu}$; this is often satisfied in practice \citep{gandhi2012autoscale, mao2012performance,mogul2015inferring, maheshwari2018scalability, hao2021empirical}.
Second, we assume that, on average, the system utilizes at least 100 servers, i.e. the offered load $R\triangleq k\rho\geq 100$.
Note also that, while these conditions are often satisfied in practice, the specific $100$ value stated here is not strictly necessary for our analysis to be accurate, as evidenced by the apparent accuracy of Approximation~\ref{apx:only}, shown in Figure~\ref{fig:approxEval}.


\newcommand{\UBone}{C_2 \left(\setuptime\right) \frac{}}
\newcommand{\shs}{\sqrt{\mu \beta R}}
\newcommand{\virt}{M}

\subsection{Upper Bound: Statement}\label{sec:upper-statement}

\begin{theorem}[Upper Bound on Average Queue Length]\label{thm:main}
For an M/M/k/Setup-Deterministic with an offered load $R \triangleq k \rho \geq 100$ and a setup time $\setuptime \geq 100 \frac{1}{\mu}$,
the expected number of jobs in queue in steady state is upper-bounded as
\begin{align*}
    \ex{Q(\infty)} 
    &\leq 3.6\sqrt{\mu \beta R} + 2.04 \frac{\rho}{1-\rho} + \frac{4.05\mu \beta^2 \sqrt{R} + g\left(9 (\mu  \beta)^2 R, 3 \mu \beta \sqrt{R}, k(1-\rho)\right)}{\beta + \frac{L_1 \mu \beta \sqrt{R}}{\mu k(1-\rho)}},
\end{align*}
where the function $g(x,y,z) \triangleq  x \frac{1}{2\mu z} + y\left[\frac{R}{\mu z^2} + \frac{3}{2 \mu z} \right]$ and the constant $L_1 = \frac{2}{3}\sqrt{\frac{\pi}{2}}$.
\end{theorem}

\subsection{Lower Bound: Statement}\label{sec:lower-statement}

\begin{restatable}[Improved Lower Bound on Average Queue Length]{theorem}{improvement}\label{thm:improvement}
    For an M/M/k/Setup-Deterministic with an offered load $R \triangleq k \rho \geq 100$ and a setup time $\setuptime \geq 100 \frac{1}{\mu}$, the expected number of jobs in queue in steady state is lower-bounded as
    \begin{equation*}
        \ex{Q(\infty)} \geq 
        \frac{ 
            L_1 \beta^2 \sqrt{R} 
            + 
            \ibp{\left[L_1 \beta \sqrt{R} - (k-R) \right]^+}{k - R}
        }
        {
           2.08 \beta +
             \frac{1}{\mu}\frac{F_1 \beta \sqrt{R}}{k - R} + 
             \frac{1}{\mu}\frac{3}{2}\ln(\beta) + \frac{1}{\mu}\ln(F_1 D_1)
        +
        \frac{2}{\mu} 
        + \frac{1}{\mu}\left[D_2 + \frac{D_3}{\sqrt{R}} \right]\max\left(\frac{1}{D_1 \sqrt{\mu \beta}}, \frac{1}{\sqrt{R}}\right)
        },
    \end{equation*}
     where $L_1$, $F_1$, $D_1$, $D_2$, and $D_3$ are constants independent of system parameters. 
\end{restatable}

\subsection{Discussion of Bounds}\label{sec:discussion_of_bnds}
After simplification, our bounds become
\begin{equation*}
    \ex{Q(\infty)} =_c  \mu \beta \sqrt{R} + \frac{1}{1-\rho};
\end{equation*}
where the operator $=_c$ denotes equality up to multiplicative constants; we show this explicitly in Section~\ref{sec:tightness}. 

This simplified characterization of the queue length gives us insight into how the system parameters govern the system's queueing behavior.
The first term, $\mu\beta \sqrt{R}$, scales linearly with the setup time $\beta$ and captures the effect of turning servers \emph{off} and \emph{on}.
The second term, $\frac{1}{1-\rho}$, dominates the first term only when the load $\rho$ is high enough, say in the renowned super-Halfin-Whitt regime \citep{HalWhi_81,LiuYin_22} where $\rho = 1-\gamma k^{-\alpha}$ with $0<\gamma<1$ and $\alpha >0.5$.
In this case, it recovers the $\frac{1}{1-\rho}$ scaling seen in the M/M/k without setup times.


% The second term, the $\frac{1}{1-\rho}$ term, captures the effect of resource contention.
% In particular, unless the load is very high, i.e. unless $\rho > 1 - \frac{1}{\mu \beta \sqrt{R}}$, the average queue length is predominantly determined by the presence of setup times.
% However, once the load is high enough, then we recover the $\frac{1}{1-\rho}$ scaling seen in the M/M/k without setup times.

    
%     However, if we increase the 
%     However, the price we end up paying for d
% - seutp time term exists in single server as well
%     - in SS, the analogous term would be the setup time multiplied by the full arrival rate, since the sys loses all of its cap when turning serv off

%     - in MS, instead of regularly losing all of our cap, we (on average), only ever lose sqrt{R} of our capacity


% goal of section: describe what's going on in the bounds in a more approachable way.
% thesis: two parts tell us a lot about how the system behaves
%     - First part tells us that setup scales linearly with the the setup time
% -   
%     - similar to the term seen in m/m/k when the system is in qed regime,  cite
%     - note that this holds regardless of how underloaded the system actually us; i.e. if load 
%     - in a sense, this is exactly what we want 

% These two terms give us good insight into precisely how setup time hurts queueing performance.
% I
%     increase k without increasing arrival rate, unless the system is near-overload (1-\rho \approx \frac{1}{\beta{\sqrt{R}}}), then adding servers doesn't help
%     (the system artificially constrains its resources) => increasing k won't help)
%     (dominant term unless very heavily loaded is caused by setup times, and scales linearly with the setup time, just like in SS)
%     (when load is high, however, the second term dominates; in fact, we recover (up to constants) the queueing behavior of the typical M/M/k)
%     in some sense, t


% The second term, $\frac{1}{1-\rho}$, scales like $\frac{1}{1-\rho}$ and captures the queueing caused by \textit{resource contention}.
% This term is reminiscent of the $\frac{1}{1-\rho}$ scaling seen in the M/M/k queue when the load is high, i.e. in the Halfin-Whitt and super-Halfin-Whitt regimes. 
% Note thou


% \subsection{Approximation: Statement and Evaluation}\label{sec:apx_statement}

% \begin{restatable}[Approximation of the Average Queue Length]{apprx}{ourapx}\label{apx:only}
%     Let $\capx \triangleq \sqrt{\frac{\pi}{2}}$. Then, if the offered load $R > 2$, one can approximate the steady state queue length as
%     \begin{equation}\label{eq:full}
%         \ex{Q(\infty)} \approx Q_{\textup{apx}} \triangleq 
%         \frac{
%             \frac{1}{2} \mu \beta^2 \capx \sqrt{R} + 
%             \frac{\mu \beta \capx \sqrt{R}} {\mu k(1-\rho)}
%             \left[
%                 \frac{\mu \beta \capx \sqrt{R} + 1}{2} + \frac{1}{1-\rho}
%             \right]
%         }
%         {
%             \beta + \frac{\mu \beta \capx \sqrt{R} }{\mu k (1-\rho)}
%         }.
%     \end{equation}
% \end{restatable}

% \begin{figure}
%     \centering
%     \includegraphics[ trim={1cm 1cm 0 0},clip, width=0.9\textwidth]{figures/multi_sweep_ss_inc.pdf}
%     \caption{Simulation results demonstrating the high accuracy of Approximation~\ref{apx:only}. For each of these 9 plots, we plot the behavior of the average waiting time as one varies the load $\rho$ from $0$ to $1$, holding fixed the total number of servers $k$ as well as the setup time $\beta$. In each row, we hold the number of servers $k$ constant while testing increasing values of the setup times $\beta$. In each column, we hold the setup time $\beta$ constant while increasing the number of servers. We plot three quantities: 1) in black, the simulated average waiting time for the M/M/k/Setup-Deterministic; 2)in purple, the predicted average waiting time of Approximation~\ref{apx:only}; and \chmade{3) the predicted average waiting time of as given by the ``low-R'' approximation of \eqref{eq:ss_approx}, a variation on the single-server setup result of \cite{welchfirstservice}.  We also include, as a reference, a dotted line illustrating the point at which the offered load $R\triangleq k\rho = 1$. Our approximation works well when the average number of busy servers $R > 1$, and the ``low-R'' approximation works well when $R < 1$.}}
% \label{fig:approxEval}
% \end{figure}

% \paragraph{Evaluation.} 
% %Our third and final result is Approximation~\ref{apx:only}.
% In Figure~\ref{fig:approxEval}, we observe that our approximation is accurate across a wide range of system parameters, so long as the offered load $R > 1$, a considerable weakening of the assumptions used in our proofs.
% In that sense, it serves as a testament to the strength of our approach that our resulting approximation remains accurate all the way down to offered loads $R < 1$.
% And, while offered loads $R < 1$ are of limited practical interest, when the offered load is that small, we anticipate that the waiting time exhibits a ``single-server bottleneck'' effect, mirroring the behavior in \citep{welchfirstservice}. 
% \chmade{
% In particular, in the M/M/1/Setup-Deterministic, one finds in \citep{welchfirstservice} that
% \begin{equation*}
%     \ex{T_Q} = \frac{1}{\mu - \lambda} + \frac{\beta}{2}\left[\frac{2 + \lambda \beta}{1 + \lambda \beta}\right].
% \end{equation*}
% Taking the second term, which measures the additional wait in the system due to setup times, and using $R$ in place of $\frac{\lambda}{\mu}$, we obtain a ``low-$R$'' approximation
% \begin{equation}\label{eq:ss_approx}
%     \ex{T_Q} \approx \frac{\beta}{2}\left[\frac{2 + \mu R \beta}{1 + \mu R \beta}\right].
% \end{equation}
% We include this ``low-R'' approximation in Figure~\ref{fig:approxEval} and note that, when $R < 1$, this approximation seems to capture the performance behavior very well.}


% For offered loads smaller than this, we anticipate that the system exhibits a ``single-server'' bottleneck effect. Preliminary investigations seem to confirm this, as, when the offered load $R<2$, the additional delay from setup observed in the multiserver setting becomes close to the additional delay from setup found in the single server setting.



% \begin{theorem}\label{thm:main}
% Let the reserve capacity $\virt$ be defined as
% $$\virt \triangleq \min\left(C_1 \shs, k - R\right)$$ for some constant $C_1$ independent of system parameters. Then, for an M/M/k/Setup-Deterministic with an offered load $R \triangleq k \rho \geq 100$ and a setup time $\setuptime \geq 1000 \frac{1}{\mu}$,
% \begin{equation*}
%     \ex{Q(\infty)} \leq A_1 \shs +
%     \frac{
%    A_2  \setuptime^2  \mu \sqrt{R} + \ibp{A_3  \setuptime \mu \sqrt{R}}{\virt} + A_4 \ibp{\virt}{\virt}
%     }
%     {
%         \setuptime + \bp{L_1 \beta \mu \sqrt{R}}{ k - R} - \frac{1}{\mu}
%     }.
% \end{equation*}
% \end{theorem}

% \wwcomment{I moved the remarks below out of the remark environment.}
%\begin{remark}\label{rem:main}



%\end{remark}




==> 999_approximation.tex <==
% \newcommand{\capx}{C_{\textup{apx}}}
\newcommand{\qapx}{Q_{\textup{apx}}}
In Section~\ref{sec:approx}, we present our approximation for the average waiting time in the M/M/k/Setup-Deterministic. We begin by discussing why we need such an approximation, then state the approximation, then give a short justification for its form.

\subsection{Why we need an approximation}

Despite our success in analyzing the M/M/$k$/Setup-Deterministic, our upper and lower bounds \emph{alone} are not suitable for practical use in predicting the value of the average waiting time $\ex{T_Q}$.

 There are two reasons for this.
 First, although we can prove that our bounds are both within a constant factor of the true waiting time (Theorem~\ref{thm:tightness}), it's not \textit{a priori} obvious whether the true value of $\ex{T_Q}$ will get closer to one bound or the other as we vary the system parameters.
 Although the true value does not \emph{seem} to ever get closer to a particular bound (and so we could conceivably just scale our lower bound to serve as a predictor), it would be better to have a more concrete theoretical justification for our prediction.

 The second reason why our bounds are unsuitable 
 % for practical use 
 is their complexity.
 Although both the upper and lower bounds are far more straightforward to compute than, for example, the average waiting time in the M/M/k/Setup-Exponential, both bounds incorporate a large number of terms and are thus somewhat difficult to reason about. % on the fly.
 %As such, it would be better to have 
 We need a predictor which incorporates only a few, easy-to-remember terms.


\subsection{Approximation: Statement}

To this end, we introduce the following approximation; the justification for the approximation follows. We evaluate the approximation in Figure~\ref{fig:approxEval}; it is extremely accurate, across a variety of parameter settings.


\begin{apprx}[Approximation to the average queue length.]\label{apx:state}
In the M/M/$k$/Setup-Deterministic, for offered loads $R\triangleq k \rho > 2$ and taking $\capx \triangleq \sqrt{\frac{\pi}{2}}$, 
\begin{equation}\label{eq:basic_appx}
    \ex{Q(\infty)} \approx \qapx \triangleq
    \frac{
        \frac{1}{2} \beta^2 \capx \sqrt{R} + \frac{\beta \capx \sqrt{R}}{\mu k(1-\rho)}\left[\frac{\beta \capx \sqrt{R} + 1}{2} + \frac{1}{1-\rho} \right]
    }
    {
        \beta + \frac{\beta \capx \sqrt{R}}{\mu k (1-\rho)}
    }.
\end{equation}

% Furthermore, when $R$ is small, the average queue length $\ex{Q(\infty)}$ becomes the minimum between the expression in \eqref{eq:basic_appx} and the ``setup penalty'' seen in the single server system,
% \begin{equation}\label{eq:single_serv_appx}
%     \ex{Q(\infty)} \leq \min\left(\qapx, \frac{\beta}{2}\left[\frac{2 + \mu \beta R}{1 + \mu \beta R} \right] \right).
% \end{equation}
\end{apprx}



\subsection{Justification}

We arrive at this bound via a straightforward combination of the bounds from Theorems~\ref{thm:main} and~\ref{thm:improvement}, along with a few modifications.
We follow our renewal-reward analysis, separately approximating the expected time integral over our renewal cycle and the expected length of that renewal cycle, which represent the numerator and denominator of (\ref{eq:basic_appx}), respectively. 

\subsubsection{Justification of Numerator.}\label{sec:approxNum}

We first approximate the 
%numerator of our expression, the 
expected time integral over our chosen renewal cycle.
We begin by recalling the lower bound on the time integral, Lemma~\ref{lem:LBint}, which states
\begin{align*}
    \ex{\int_0^{\cycle}{Q(t) \dd t}} \geq    L_1 \beta^2 \sqrt{R} 
            + 
            \ibp{\left[L_1 \beta \sqrt{R} - (k-R) \right]^+}{k - R},
\end{align*}
where $$\ibp{x}{z} \triangleq \frac{x}{\mu z} \left[\frac{x+1}{2} + \frac{1}{1-\frac{k\lambda}{k\lambda + \mu z}}\right]$$ represents the time integral of the queue length a certain M/M/1 queue over a busy period started by $x$ jobs. 

To obtain the appropriate constant $\capx$, we next note that, although our theorem states $L_1$ as an absolute constant, as the setup time $\beta$ and the offered load $R$ grow, the best possible constant will become $\capx = \sqrt{\frac{\pi}{2}}$. Under the hood, this convergence stems from the fact that
\begin{equation*}
    \sum_{j=1}^{R}{\prod_{i=1}^{j}{\left(1-\frac{j}{R}\right)}} \approx \int_0^{\infty}{e^{\frac{-j^2}{2R}}\dd j} = \frac{1}{2} \sqrt{2 \pi R};
\end{equation*}
see the proof of Lemma~\ref{lem:LBint} for more details. 

To complete the approximation, it suffices to remove the subtraction of $(k-R)$ in the busy period term, which we anticipate is an artifact of our analysis. Removing it, we obtain the desired approximation 
\begin{equation}\label{eq:approxNum}
    \ex{\int_0^{X}{Q(t)\dd t}} \approx  \frac{1}{2} \beta^2 \capx \sqrt{R} + \frac{\beta \capx \sqrt{R}}{\mu k(1-\rho)}\left[\frac{\beta \capx \sqrt{R} + 1}{2} + \frac{1}{1-\rho} \right].
\end{equation}

\subsubsection{Justification of Denominator.}

We next approximate the denominator of our expression, the expected length of our chosen renewal cycle.
To do so, we again make use of the lower bound on the expected cycle length $\ex{X}$ from Lemma~\ref{lem:LBX}, which states
\begin{equation*}
    \ex{X} \geq \beta + \frac{L_1 \beta \sqrt{R}}{\mu k(1-\rho)}.
\end{equation*}
By making the same convergence argument for $L_1$, i.e. that $L_1 \to \capx$ for large setup times $\beta$ and large offered loads $R$, we obtain the denominator, completing both parts of our bound.





==> ThesisFiles/UB/thm_UB.tex <==


We now describe the full proof of Theorem~\ref{thm:upbnd}. As discussed in Chapter~\ref{ch:tech}, it suffices to prove the three following lemmas.

\begin{restatable}[Accumulation Period Upper Bound]{lemma}{mainone}\label{lem:UBintTA}
Suppose the system begins at time $0$ with $R$ jobs in service and no jobs in the queue (and thus no servers in setup), and define the accumulation time $$T_A \triangleq \minpar{t \geq 0: Z(t) = R+1}$$ to be the moment the $(R+1)$-th server turns on.

Then,
	\begin{equation*}
		\ex{\int_0^{T_A}{[N(t) - R] \dd t}} \leq B_1 \shs \cdot \ex{T_A} + B_2 \beta^2 \mu \sqrt{R},
	\end{equation*}
where $B_1 = 3.6$ and $B_2 = 1.04$.
\end{restatable}

\begin{restatable}[Draining Period Upper Bound]{lemma}{maintwo}\label{lem:UBintTB}
Recall that accumulation time $T_A$ is the first (and only) time the $(R+1)$-th server turns on during a renewal cycle, and that the next renewal point $X = \minpar{t > T_A: Z(t) = R}$ is simply the next time the $(R+1)$-th server turns off. 
Then, 
	\begin{align*}
	&\ex{\int_{T_A}^{X}{[N(t) - R]^+ \dd t}}\\
    &\;\; \leq \left(B_5 \shs + B_6 \mu \beta \sqrt{R}\right)\cdot \beta + \ibp{B_5 \shs + B_6 \mu \beta \sqrt{R}}{M} + B_7\frac{\beta R}{M}\\
    &\;\; + \left[ 2M + 2\frac{R}{M}\right] \ex{X-T_A} +  \frac{1}{1-p_2}\ibp{M}{M},
	\end{align*}
 where all of these quantities are defined in Chapter~\ref{ch:model} and Section~\ref{sec:taexpect}.
\end{restatable}

\begin{restatable}[Cycle Length Lower Bound]{lemma}{mainthree}\label{lem:LBX}
Suppose the system begins at time $0$ with $R$ jobs in service and no jobs in the queue (and thus no servers in setup), and let $$X \triangleq \minpar{t > 0: Z(t^-) =  R+1, Z(t) = R}$$ be the next time the $(R+1)$-th server turns off.

	Then,
	\begin{equation*}
		\ex{X} \geq \setuptime + \bp{D_1 \beta \mu \sqrt{R}}{ k - R},
	\end{equation*}
 where $D_1$ is a constant independent of system parameters.
\end{restatable}
% \wwcomment{We sometimes say ``absolute constant'' and sometimes say ``constants independent of system parameters''.  It might be good to unify them.}

After proving these lemmas, the result follows by a bit of algebra. First, note that, by summing the two integral bounds, one obtains
\begin{align*}
    &\ex{\int_0^X{[N(t) - R] \dd t}}\\
    &\;\;\leq B_1 \shs \cdot \ex{T_A} + B_2 \beta^2 \mu \sqrt{R} + \left(B_5 \shs + B_6 \mu \beta \sqrt{R}\right)\cdot \beta\\
    &\;\; + \ibp{B_5 \shs + B_6 \mu \beta \sqrt{R}}{M} + B_7\frac{\beta R}{M} + \left[ 2M + 2\frac{R}{M}\right] \ex{X-T_A} +  \frac{1}{1-p_2}\ibp{M}{M}\\
    &\;\;\leq B_1 \shs \cdot \ex{T_A} + B_2 \beta^2 \mu \sqrt{R} + \left(B_5 \shs\right)\ex{T_A} + B_6 \mu \beta^2 \sqrt{R}\\
    &\;\; + \ibp{B_5 \shs + B_6 \mu \beta \sqrt{R}}{M} + B_7\frac{R}{M}\ex{T_A} + \left[ 2M + 2\frac{R}{M}\right] \ex{X-T_A} +  \frac{1}{1-p_2}\ibp{M}{M}\\
    &\;\;\leq \max\left(2M + 2 \frac{R}{M}, (B_1 +B_5) \shs + B_7 \frac{R}{M} \right) \ex{X} + (B_2+B_6) \beta^2 \mu \sqrt{R}\\
    &\;\; + \ibp{B_5 \shs + B_6 \mu \beta \sqrt{R}}{M} + \frac{1}{1-p_2}\ibp{M}{M}\\
    &= \left(A_1 \shs + A_2 \frac{R}{M}\right)\ex{X} + A_3\beta^2  \mu \sqrt{R} + \ibp{B_5 \shs + B_6 \mu \beta \sqrt{R}}{M} + A_4 \ibp{M}{M},
\end{align*}
where we have taken the constant $A_1 \triangleq \max{\left(B_1+B_5, C_3\right)}$, the constant $A_2 \triangleq B_2 + B_3$, the constant $A_3 \triangleq B_2 + B_6$, and the constant $A_4 = \frac{1}{1-p_2}$. Upon dividing the reward integral by the cycle length, we obtain that
\begin{align*}
    \ex{Q(\infty)} &= \frac{\ex{\int_0^X{[N(t) - R] \dd t}}}  {\ex{X}}\\
    &\leq \frac{\left(A_1 \shs + A_2 \frac{R}{M}\right)\ex{X} + A_3\beta^2  \mu \sqrt{R} + \ibp{B_5 \shs + B_6 \mu \beta \sqrt{R}}{M} + A_4 \ibp{M}{M}}
        {\ex{X}}\\
    &= A_1 \shs + A_2 \frac{R}{M} + 
    \frac{A_3 \beta^2 \mu \sqrt{R} +  \ibp{B_5 \shs + B_6 \mu \beta \sqrt{R}}{M} + A_4 \ibp{M}{M}}
    {\ex{X}}\\
    &\leq A_1 \shs + A_2 \frac{R}{M} + 
    \frac{A_3 \beta^2 \mu \sqrt{R} +  \ibp{B_5 \shs + B_6 \mu \beta \sqrt{R}}{M} + A_4 \ibp{M}{M}}
    {\setuptime + \bp{D_1 \beta \mu \sqrt{R}}{ k - R}},
\end{align*}
which is the upper bound stated in Theorem~\ref{thm:upbnd}.

% Before we continue on to those proofs, we first give a formal construction of the system we analyze, then prove a few useful coupling claims.

% \wwcomment{Need to resolve the numbering issue with the restate environment.}

% \input{coupling_construction}







\input{UB/lemma_UB_int_TA}


\input{UB/lemma_UB_int_TB}

\input{UB/lemma_LB_X}






==> acknowledgments.tex <==
This research was supported by NSF CMMI-1938909, NSF CSR-1763701, NSF CNS-200773, and NSF ECCS-2145713, in addition to the Gates Millennium and GEM Fellowships.

==> claims/dcbnds.tex <==
\newcommand{\dgen}{\gamma}
\newcommand{\filt}[1]{\mathcal{F}_{#1}}


\begin{restatable}{claim}{dcbnd}\label{clm:dcint}
    Let $\tau$ be some stopping time. Let the next down-crossing $\dgen$, defined as
    \begin{equation*}
        \dgen \triangleq \minpar{t \geq 0: N(t + \tau) \leq h},
    \end{equation*}
    be the amount of time that passes before the number of jobs $N(t)$ is less than some fixed threshold $h$. Suppose that, at time $\tau$, we have a lower bound on the number of busy servers over a period, i.e.
    \begin{equation*}
        Z(t) \geq R - j,
    \end{equation*}
    for all $t \in \left[\tau, \tau + \mintwo{\ell}{\dgen} \right]$ and for some non-negative $j$. 
    Then we have the following bound on the integral over this time period:
    \begin{equation*}
        \ex{\int_{\tau}^{\tau + \mintwo{\dgen}{\ell}}{\left[N(t) - h\right] \dd t}\middle | \filt{\tau}} \leq \ell \cdot \left[N(\tau) - h \right]^+ + \frac{1}{2}\mu j \ell^2.
    \end{equation*}
\end{restatable}
\begin{proof}
    
\end{proof}



\begin{restatable}{claim}{dcprob}\label{clm:dcprob}
    Let $\tau$ be some stopping time. Let the next down-crossing $\dgen$, defined as
    \begin{equation*}
        \dgen \triangleq \minpar{t \geq 0: N(t + \tau) \leq h},
    \end{equation*}
    be the length of time until the number of jobs $N(t)$ is less than some fixed threshold $h$.
    We consider two cases.
    
    In the first case, suppose that we have a lower bound on the number of busy servers $Z(t)$ over some length $\ell$ interval starting at time $\tau$, i.e.
        \begin{equation*}
        Z(t) \geq R - j,
    \end{equation*}
    for all $t \in \left[\tau, \tau + \mintwo{\ell}{\dgen} \right]$ and for some non-negative $j$. 
    Then, we can bound the threshold-crossing probability by
    \begin{equation*}
        \pr{\dgen < \ell\middle | \filt{\tau}} \leq 2\Phi\left(-\left[\frac{N(\tau) - h}{\sqrt{2 k\lambda \beta}}\right]\right) + \frac{2}{3\sqrt{\ell(2k\lambda - \mu j} }.
    \end{equation*}
    In particular, if $N(\tau) - h = c \sqrt{\mu \beta R}$, then
    \begin{equation*}
        \pr{\dgen < \ell\middle | \filt{\tau}} \leq 2 \Phi\left( - \frac{c_1}{\sqrt{2}} \right) + \frac{1}{100}.
    \end{equation*}

    In the second case, suppose that we instead have an upper bound on $Z(t) \leq R$ during this interval instead. Then,
    \begin{equation*}
        \pr{\dgen < \ell \middle | \filt{\tau}} \geq 2 \Phi\left(-\left[ \frac{N(\tau) - h}{\sqrt{2 \beta k \ell}}\right] \right) - \frac{2}{3\sqrt{2 k\lambda \ell}}.
    \end{equation*}
    As before, if $N(\tau) - h =  c \sqrt{\mu \beta R}$, then
    \begin{equation*}
                \pr{\dgen < \ell\middle | \filt{\tau}} \geq 2 \Phi\left( - \frac{c}{\sqrt{2}} \right) - \frac{1}{100}.
    \end{equation*}
\end{restatable}


==> theorem1/lemma1.tex <==
\newcommand{\systag}{\textup{sys}}
\newcommand{\cfoursys}{C_4^{\systag}}

\subsection{Proof of Lemma~\ref{lem:mainone}}\label{sec:lemma1}
We are now ready to begin proving our main lemmas. We start with Lemma~\ref{lem:mainone}, restated here for the reader's convenience.
\mainone*

We prove this result via two applications of Lemma~\ref{lem:waldstop}. To apply this decomposition lemma, there are two broad steps. First, we must specify a starting stopping time ($T_0$), an ending stopping time ($P$), a series of intervening stopping times $(T_i)$, the process ($Y_t$), and an counting variable ($F$). Second, we must prove that the three preconditions of the lemma hold, given these specifications. 

\subsubsection{First Application of Lemma~\ref{lem:waldstop}}

\paragraph{Definition of $(\tau_j)$.} As outlined in Section~\ref{sec:keyideas}, we define the sequence of stopping times $(\tau_j: j=0,1,\dots, R)$ as
\begin{equation*}
    \tau_j \triangleq \minpar{t>0: N(t) \leq R - j},
\end{equation*}
i.e., $\tau_j$ is the first time there are only $R-j$ jobs within the system. Note that, by definition, $\tau_0 = 0$. We call the period $\bigg [\tau_j, \mint{\tau_{j+1}}{T_A} \bigg )$ the \emph{$j$-th epoch}, and say epoch $j$ occurs whenever $\tau_j < T_A$. We then let the random variable $\epochind$ denote the number of epochs which occur in a given renewal cycle.

\paragraph{Specification Step.} Since we are interested in bounding $\ex{\int_0^{T_A}{[N(t) - R] \dd t}}$, we let our starting stopping time be $T_0 = 0$, our ending stopping time be $P=T_A$, our intervening stopping times be $T_j = \tau_j$, the process of interest $Y_t = N(t) - R$ and our counting variable be $F=\epochind$. Let $$\prise{j} \triangleq \pr{\max_{t \in [\tau_j, \mintwo{\tau_{j+1}}{T_A}}{N(t)} \geq R + C_3\shs \middle | \epochind \geq j}$$ be the probability that the total number of jobs $N(t)$ exceeds $R+ \threshone$ during epoch $j$. From here, to apply Lemma~\ref{lem:waldstop}, it suffices to show the following claims: %\wwcomment{Please change the names of the claims to something with more semantic meaning.}
\begin{restatable}[Accumulation Phase, Integral Bound]{claim}{aone}\label{clm:a1}
Let $\tau_j \triangleq \minpar{t\geq0: N(t) \leq R - j}$, $T_A \triangleq \minpar{t \geq0: Z(t) = R+1}$, and let $\epochind \triangleq \maxpar{i\in \zplus: \tau_i < T_A}$. Then,
    \begin{equation*}
        \ex{\int_{\tau_j}^{\mintwo{\tau_{j+1}}{T_A}}{[N(t) - R] \dd t}\middle | \epochind \geq j} \leq B_1 \shs \cdot \ex{\mintwo{\tau_{j+1}}{T_A} - \tau_j \middle | \epochind \geq j} + C_2 \beta^2 \mu j \prise{j} ,
    \end{equation*}
    where $B_1=3.6$ and $C_2= \frac{1}{2\cdot 0.98} < 0.511$.
\end{restatable}

\begin{restatable}[Accumulation Phase, Continuing Probability Bound]{claim}{atwo}\label{clm:a2}
 Recall that the total number of epochs $\epochind \triangleq \maxpar{j\in \zplus: \tau_j < T_A}$. Then,
    \begin{equation*}
        \pr{ \epochind \geq j+1 \middle | \epochind \geq j} \leq 1 - C_4\prise{j}, 
    \end{equation*}
    where $C_4= 0.98$.
\end{restatable}

%\wwcomment{I added a heading to make the structure clearer.}

\subsubsection*{Proof of Lemma~\ref{lem:mainone} assuming Claims~\ref{clm:a1} and \ref{clm:a2}.}
Before going further, we show how to complete the proof of Lemma~\ref{lem:mainone}, assuming the two prior claims. Applying Lemma~\ref{lem:waldstop}, we find that
\begin{align*}
    \ex{\int_0^{T_A}{[N(t) - R] \dd t}} &\leq B_1 \shs \cdot \ex{T_A} + C_2 \beta^2 \mu \sum_{j=1}^{R}{j \prise{j} \prod_{i=1}^{j-1}{\left(1 - C_4 \prise{j} \right)}}\\
    &\leq B_1 \shs \cdot \ex{T_A} + \frac{C_2}{C_4} \beta^2 \mu \left[\sum_{j=1}^{R}{j C_4 \prise{j} \prod_{i=1}^{j-1}{\left(1 - C_4 \prise{j} \right)}} \right]\\
    &= B_1 \shs \cdot \ex{T_A} + \frac{C_2}{C_4} \beta^2 \mu \left[\sum_{j=1}^{R}{\prod_{i=1}^{j}{\left(1 - C_4 \prise{j} \right)}} \right],
\end{align*}
where we have made use of the ``expectation as a sum of tails'' trick in the final line. From here, we make use of the following claim:
\begin{restatable}{claim}{prisebnd}\label{clm:prisebnd}
    Let $\prise{j} \triangleq \pr{\max_{t \in [\tau_j, \mintwo{\tau_{j+1}}{T_A}}{N(t)} \geq R + C_3\shs \middle | \epochind \geq j}$ be the probability that the total number of jobs $N(t)$ exceeds $R+ \threshone$ during epoch $j$. Then, for $j \geq A_5 \sqrt{R}$,
    \begin{equation*}
        \prise{j} \geq 0.99\frac{A_5}{\sqrt{R}}.
    \end{equation*}
\end{restatable}
We defer the proof of Claim~\ref{clm:prisebnd} to Section~\ref{sec:prisebnd}. Applying the claim's result, we find that
\begin{align*}
    \sum_{j=1}^{R}{\prod_{i=1}^{j}{\left(1 - C_4 \prise{j} \right)}} &\leq  \sum_{j=1}^{R}{\left(1 - \frac{0.99 C_4 A_5}{\sqrt{R}}\right)^{[j - A_5 \sqrt{R}]^+}}\\
    &\leq \sum_{j=1}^{\infty}{\left(1 - \frac{0.99 C_4 A_5}{\sqrt{R}}\right)^{[j - A_5 \sqrt{R}]^+}}\\
    &= A_5 \sqrt{R} + \sum_{j=0}^{\infty}{\left(1 - \frac{0.99 C_4 A_5}{\sqrt{R}}\right)^j}\\
    &= A_5 \sqrt{R} + \frac{1}{0.99 C_4 A_5} \sqrt{R}
\end{align*}
Returning to our original inequality, we obtain that
\begin{align*}
    \ex{\int_0^{T_A}{[N(t) - R] \dd t}} \leq B_1 \shs \cdot \ex{T_A} + \frac{C_2}{C_4}\left( A_5 + \frac{1}{0.99 C_4 A_5}\right) \beta^2 \mu \sqrt{R}.
\end{align*}
Noting that $A_5 =  1$ and taking $B_2\triangleq 1.04 > \frac{C_2}{C_4}\left( A_5 + \frac{1}{0.99 C_4 A_5}\right)$, the proof is complete. \hfill \Halmos

And so, assuming the preconditions of Lemma~\ref{fig:waldstop} (Claim~\ref{clm:a1} and Claim~\ref{clm:a2}) as well as a few helper claims, we have proven Lemma~\ref{lem:mainone}. Thus, it now suffices to prove those preconditions. 

\subsubsection{Proof of Claim~\ref{clm:a2}.} Proving Claim~\ref{clm:a1} will be more involved; we deal with Claim~\ref{clm:a2} first. 
Note that 
\begin{align*}
    \pr{ \epochind \geq j+1 \middle | \epochind \geq j} &= 1 - \pr{\epochind = j \middle | \epochind \geq j}\\
    &= 1 - \pr{T_A < \tau_{j+1} \middle | \epochind \geq j}.
\end{align*}
Thus, it suffices to show that
\begin{equation*}
    \pr{T_A < \tau_{j+1} \middle | \epochind \geq j} \geq C_4 \prise{j}.
\end{equation*}
To do this, we note a particular sequence of events which results in $T_A < \tau_{j+1}$. In particular, we define the up-crossing time $u =\minpar{t >\tau_j: N(t) \geq R+\threshone}$ and the down-crossing time $d = \minpar{t > u: N(t) \leq R}$, then let $\event_1$ be the event that $\gamma < \tau_{j+1}$ and let $\event_2$ be the event that $T_A < d$.  Note also that, since jobs depart one at a time, the down-crossing time $d < \tau_{j+1}$. Thus,
\begin{equation*}
    \pr{T_A < \tau_{j+1} \middle | \epochind \geq j} \geq \pr{\event_1 \middle | \epochind \geq j} \pr{\event_2 \middle | E_1} = \prise{j} \pr{\event_2 \middle | E_1}.
\end{equation*}
To bound $\pr{\event_2 \middle | E_1}$, we couple our original number of jobs $N(t)$ to a coupled number of jobs $\ncouple(t)$. We construct $\ncouple(t)$ as
\begin{equation*}
    \ncouple(t) \triangleq N(u) + \Pi_A\left( (u, t] \right) - \depOp{R}{(u, t]},
\end{equation*}
where $t \in \bigg [u, \mintwo{d}{T_A} \bigg)$. Since $Z(t) \leq R$ for all $t< T_A$, we have that $\ncouple(t) \leq N(t)$ for all $t$ in our interval. Let $\dcouple \triangleq \minpar{t>u:\ncouple(t) \geq R}$ be the analogous down-crossing time in the coupled system. Clearly, $\dcouple \leq d$. Thus, 
\begin{align*}
    \pr{T_A < \tau_{j+1} \middle | \event_1} \geq \pr{T_A < d \middle | \event_1} \geq \pr{T_A <  \dcouple \middle | \event_1}.
\end{align*}

Finally, note that, if $\dcouple > u + \setuptime$, then $N(t)$ must have stayed above $R$ for an entire setup time, i.e. $\dcouple < T_A$. Thus, it suffices to show that
\begin{equation*}
    \pr{\dcouple - u >  \setuptime} \geq C_4.
\end{equation*}
We prove this with a straightforward application of Claim~\ref{clm:dcprob}. In particular, since we know the number of busy servers $Z(t) \leq R$ for any time before $T_A$, we can apply the second case and see that
\begin{equation*}
    \pr{\dcouple - u > \setuptime} \geq 1 - 2\Phi\left(-\frac{C_3}{\sqrt{2}}\right) - \frac{2}{3\sqrt{ \mu \beta R}}\geq 0.98
\end{equation*}
Taking this to be $C_4$, we have completed our proof. \hfill \Halmos

\subsubsection{Proof of Claim~\ref{clm:a1}}\label{sub:updown}
With the probability claim proven, we return to the proving Claim~\ref{clm:a1}, the upper bound on the time integral over an epoch.
As discussed previously, we do this via another application of Lemma~\ref{lem:waldstop}; we specify the stopping times being used, then prove that the preconditions hold. Before the specification step, though, we must define a paired sequence of stopping times, which we call up-crossings and down-crossings.

\begin{figure}
    \centering
    \includegraphics[scale=0.32,clip]{figures/up_down_new.pdf}
    \caption{A depiction of the up-crossings and down-crossings defined in Section~\ref{sub:updown}. In this example, we see that the number of up-crossings in epoch $3$ is $\epochind(3) = 2$ and that, in this case, epoch $3$ ends when epoch $4$ begins (i.e. at time $\tau_4$).}
    \label{fig:updown}
\end{figure}


\paragraph{Definition of Up-crossings and Down-Crossings.} Let the $0$-th down-crossing time in epoch $j$ occur at time $\tau_j$, i.e. 
\begin{equation*}
    d_0^{(j)} \triangleq \tau_j.
\end{equation*}
Next, define the first up-crossing in epoch $j$ as the first time during epoch $j$ that the total number of jobs $N(t)$ exceeds $R+ \threshone$, i.e.
\begin{equation*}
    u_1^{(j)} \triangleq \minpar{t > \tau_j : N(t) \geq R + \threshone}.
\end{equation*}
From here, define $i$-th down-crossing in epoch $j$ and the $i+1$-th up-crossing in epoch $j$ as
\begin{equation*}
    d_i^{(j)} \triangleq \minpar{t \geq u_i^{(j)} : N(t) \leq R}
\end{equation*}
and
\begin{equation*}
    u_{i+1}^{(j)} \triangleq \minpar{t \geq d_i^{(j)} : N(t) \geq R+ \threshone},
\end{equation*}
respectively; we visualize these definitions in Figure~\ref{fig:updown}. We call the interval $\bigg [ d_i^{(j)}, \mintwo{u_i^{(j)}}{\mintwo{T_A}{\tau_{j+1}}} \bigg)$ the $i$-th rise, and the interval $\bigg [u_i^{(j)}, \mintwo{d_i^{(j)}}{\mintwo{T_A}{\tau_{j+1}}}\bigg)$ the $i$-th fall.  We say the $i$-th up-crossing occurs if $u_i^{(j)} < \mintwo{T_A}{\tau_{j+1}}$ and let $$\upind \triangleq \maxpar{i \geq 0: u_i^{(j)}} < \mintwo{\tau_{j+1}}{T_A}$$ be the random number of up-crossings which occur in epoch $j$. Note that, if the $i$-th up-crossing occurs, then, by definition, $d_i < \tau_{j+1}$; this means that the $i$-th fall can always be written as $\bigg[u_i, \mintwo{T_A}{d_i} \bigg )$. For readability, we fix our epoch of interest and omit the superscript $j$ on our up-crossings and down-crossings.


\paragraph{Specification Step.} With up-crossings and down-crossings defined, we are now ready to specify our application of Lemma~\ref{lem:waldstop}. We let our starting stopping time be $T_0 = \tau_j = d_0$, our ending stopping time be $P = \mintwo{T_A}{ \tau_{j+1}}$, our intervening sequence be $\left(u_i\right)_{i=1}^{\infty}$, our process of interest be $[N(t) - R]$, and our counting variable be $F = \epochind$. From here, in order to apply Lemma~\ref{lem:waldstop}, we must show the following three claims:

\begin{restatable}[Within Epoch, Initial Integral Bound]{claim}{aonei}\label{clm:aonei}
    One can bound the initial integral by
\begin{equation*}
        \ex{\int_{d_0}^{\mintwo{u_1}{\mintwo{T_A}{\tau_{j+1}}}}{[N(t) - R] \dd t} \middle | \epochind \geq j} \leq B_1  \shs \cdot \ex{\mintwo{u_1}{\mintwo{T_A}{\tau_{j+1}}} - \tau_j \middle | \epochind \geq j},
\end{equation*}
where $B_1 = 3.6$.
\end{restatable}

\begin{restatable}[Within Epoch, Continuing Integral Bound]{claim}{aoneii}\label{clm:aoneii}
    One can bound the intervening sequence integrals by
\begin{align*}
      \ex{\int_{u_i}^{\mintwo{u_{i+1}}{\mintwo{T_A}{\tau_{j+1}}}}{[N(t) - R] \dd t} \middle | \upind \geq i} &\leq B_1 \shs \cdot  \ex{\mintwo{u_{i+1}}{\mintwo{T_A}{\tau_{j+1}}} - u_i \middle | \upind \geq i} \\
      &\;\;\;\; + r_1 \beta^2 \mu j,
\end{align*}
where $r_1 =  \frac{1}{2}$ is an absolute constant independent of system parameters.
\end{restatable}

\begin{restatable}[Within Epoch, Continuing Probability Bound]{claim}{aoneiii}\label{clm:aoneiii}
    Recall that $\prise{j}$ is the probability that the total number of jobs $N(t)$ ever exceeds $R + \threshone$ during epoch $j$, given that epoch $j$ occurs. Then,
    \begin{equation*}
        \pr{\upind > 0} = \prise{j}
    \end{equation*}
    and, for all $i \geq 1$,
    \begin{equation*}
        \pr{\upind \geq i+1 \middle | \upind \geq i} \leq 0.02 = (1 - p_2),
    \end{equation*}
    where $p_2$ is an absolute constant independent of system parameters.
\end{restatable}

Once again, before we move on to the proofs of these claims, we show that they indeed suffice to prove our goal, Claim~\ref{clm:a1}. By Lemma~\ref{lem:waldstop},
\begin{align*}
    \ex{\int_{\tau_j}^{\mintwo{T_A}{\tau_{j+1}}}{[N(t) - R] \dd t}\middle | \epochind \geq j} &\leq B_1  \shs \cdot \ex{{\mintwo{T_A}{\tau_{j+1}}} - \tau_j \middle | \epochind \geq j}\\
    &\;\;\;\; + \prise{j} r_1 \beta^2 \mu j \sum_{i=1}^{\infty}{   \left(1 - p_2\right)^{i-1}}\\
    &= B_1  \shs \cdot \ex{{\mintwo{T_A}{\tau_{j+1}}} - \tau_j \middle | \epochind \geq j} + \prise{j} \frac{r_1}{p_2} \beta^2 \mu j,
\end{align*}
setting $C_2 \triangleq \frac{r_1}{p_2}$, we obtain Claim~\ref{clm:a1}. \hfill \Halmos

All that remains in our proof of Lemma~\ref{lem:mainone} is to show the three aforementioned claims. 
\paragraph{Proof of Claim~\ref{clm:aonei}.}
Proving this claim is quite simple. In fact, we now prove a far more general claim, that
\begin{equation}\label{eq:downbnd}
    \int_{d_i}^{\mintwo{u_i}{\mintwo{T_A}{\tau_{j+1}}}}{[N(t) - R] \dd t}\leq \threshone \cdot \left[\mintwo{T_A}{\tau_{j+1}} - d_i \right].
\end{equation}
To see this, it suffices to note that, at any point between a down-crossing and up-crossing, the total number of jobs $N(t)$ must be strictly less than $R+\threshone$. Apply this to the $0$-th down-crossing and we have the claim. \hfill \Halmos

\paragraph{Proof of Claim~\ref{clm:aoneii}.}
This proof is a bit more involved. We separate the interval $\bigg[u_i, \mintwo{u_{i+1}}{\mintwo{T_A}{\tau_{j+1}}} \bigg )$ into the $i$-th fall and the $i$-th rise, as discussed previously.  For the rising portion, we can simply apply $\eqref{eq:downbnd}$. For the falling portion, we apply the integral coupling claim, Claim~\ref{clm:dcbnd}. In particular, note that $Z(t)\geq R - j$ until time $\tau_{j+1}$ and that the interval $[u_i, \mintwo{d_i}{T_A})$ is equivalent to the interval $[u_i, \mintwo{d_i}{u_i + Y_{R+1}(u_i)})$. Applying Claim~\ref{clm:dcbnd}, we find that
\begin{align*}
    \ex{ \int_{u_i}^{\mintwo{d_i}{T_A}}{[N(t) - R] \dd t}\middle | \state(u_i)}
    &\leq  \frac{1}{2}\beta^2 \mu j + \left[N(u_i) - R\right] \cdot \rem{R+1}(u_i)\\
    &= \frac{1}{2}\beta^2 \mu j + \threshone \cdot \rem{R+1}(u_i).
\end{align*}
From here, we note that $\rem{R+1}(u_i) \leq  \mintwo{d_i}{T_A}$  with probability at least $$ \min_{S(u_i)}{\pr{d_i < T_A \middle | \upind \geq i, S(u_i)}} \geq p_2.$$ Thus,
\begin{equation*}
    \rem{R+1}(u_i) \leq \frac{1}{p_2} \ex{\mintwo{d_{i}}{T_A} - u_i \middle | \state(u_i)}.
\end{equation*}
After combining our bound on the $i$-th fall with our bound on the $i$-th rise, then taking $B_1 = \frac{C_3}{p_2}$ and $r_1 = \frac{1}{2}$, we have the claim. \hfill \Halmos

\paragraph{Proof of Claim~\ref{clm:aoneiii}.}
We now proceed to our final claim, a statement concerning the probability $\pr{\upind > 0}$ and the conditional continuation probability $\pr{\upind \geq i+1 \middle | \upind \geq i}$.

To begin, we first note that, since the first up-crossing occurs once $N(t)$ exceeds $R+\threshone$ during epoch $j$, one has 
\begin{equation*}
    \prise{j} \triangleq \pr{u_1 < \mintwo{T_A}{\tau_{j+1}}} = \pr{\upind > 0}.
\end{equation*}

Next, we note that there can only be another up-crossing after the $i$-th up-crossing in an epoch if the $i$-th down-crossing before time $T_A$, i.e.
\begin{equation*}
    \pr{\upind \geq i+1 \middle | \upind \geq i} \leq \pr{d_i < T_A \middle | \upind \geq i}.
\end{equation*}
To bound this down-crossing probability, we condition on the filtration at time $u_i$ and make a worst-case bound based on the state at that time. First, we show that
the event $\brc{d_i < T_A} = \brc{d_i < u_i + \dets_{R+1}(u_i)}$, given that the $i$-th up-crossing has occurred. To see this, note that at time $u_i$, if another down-crossing \emph{doesn't} occur before the $(R+1)$-th server turns on, we know that $T_A = u_i + \dets_{R+1}(u_i)$. Likewise, if another down-crossing \emph{does} occur before the $(R+1)$-th server turns on, then $$T_A > d_i + \setuptime > u_i + \setuptime > u_i + \dets_{R+1}(u_i).$$ 
Thus, the event $\brc{d_i < T_A} = \brc{d_i < u_i + \dets_{R+1}(u_i)}$, given that the $i$-th up-crossing has occurred.

To bound this probability, we appeal to Claim~\ref{clm:dcbnd}. 
Since we are in the first part of our renewal cycle, we know that the $(R+1)$-th server has not yet turned on, i.e. that $Z(t) \leq R$.
If we let $\gamma = d_i - u_i$, then
\begin{equation*}
	\gamma = \minpar{ t>0: N(t + u_i) \leq R},
\end{equation*}
and thus
\begin{equation*}
		\pr{ d_i < u_i + \rem{u_i} \middle | \upind \geq i} = \pr{ \gamma < \rem{u_i} \middle | \upind \geq i}.
\end{equation*}
Applying the second case of Claim~\ref{clm:dcbnd} and noting that $N(u_i) - R = \threshone$, we obtain that
\begin{equation*}
	\pr{ \gamma < \rem{u_i} \middle | \upind \geq i} \leq 2\Phi\left( -\frac{C_3}{\sqrt{2}} \right) + \frac{1}{100}< 0.02
\end{equation*}
Taking this final quantity to be $(1-p_2)$, we have the claim.
\hfill \Halmos

% \wwcomment{I'd remove this sentence.}
% Having completed our proofs of all these claims, we have thus proven Lemma~\ref{lem:mainone}. \hfill \Halmos

==> theorem1/lemma2.tex <==
\newcommand{\visit}[1]{v_{#1}}
\newcommand{\threshtwo}{C_4 \shs}
\newcommand{\vind}{n_V}

\subsection{Proof of Lemma~\ref{lem:maintwo}}\label{sub:maintwo}
We now prove our second main lemma, restated here for the reader's convenience.

\maintwo*

To prove this lemma, we again make use of Lemma~\ref{lem:waldstop}. 
We proceed through the usual two-step process, first defining the stopping time sequence we will analyze over, 
then proving the three preconditions of the lemma.

\begin{figure}
    \centering
    \includegraphics[scale=0.32,clip]{figures/sepvisits_new.pdf}
    \caption{A depiction of the separated visits defined in Section~\ref{sub:maintwo}. In this example, we find that the number of visits is $n_v = 4$. Notice that the second separated visit only happens when \emph{both} a setup time $\setuptime$ has passed \emph{and} the number of jobs $N(t)$ is currently $ \leq R+M$. For the third visit, these events happen simultaneously.}
    \label{fig:sepvisits}
\end{figure}

\paragraph{Definition of the separated visits $(v_i)$.} 
We define the first separated visit $\visit{1}$ 
as the first moment in the second phase that the number of jobs $N(t)$ dips below some threshold value $R + M$, i.e.
\begin{equation*}
	\visit{1} \triangleq \minpar{t\geq T_A: N(t) \leq R + M},
\end{equation*}
where one should recall that $M\triangleq \min\left(C_1 \shs, k - R\right)$.
From here, we define future separated visits as
\begin{equation*}
	\visit{i+1} \triangleq \minpar{ t \geq \visit{i} + \setuptime: N(t) \leq R + M};
\end{equation*}
we visualize these visits in Figure~\ref{fig:sepvisits}.
We say that the $i$-th visit occurs if $\visit{i} \leq X$, 
and define $\vind \triangleq \maxpar{i \in \zplus: \visit{i} \leq X}$ as the number of visits which occur.



\paragraph{Specification Step.}
Since we are interested in bounding $\ex{\int_{T_A}^{X}{[N(t) - R] \dd t}}$, we let our starting time $T_0 = T_A$, our ending time $P=X$, our intervening times be $T_j = \visit{j}$, the process of interest $Y_t = N(t) - R$, and our counting variable be $F = \vind$.
As before, it suffices to prove the following claims:

\begin{restatable}[Draining Phase, Initial Integral Bound]{claim}{bone}\label{clm:b1}
    One can bound the integral until the first separated visit by
    \begin{equation*}
        \ex{\int_{T_A}^{\visit{1}}{[N(t) - R] \dd t}\middle| \filt{T_A}} \leq \setuptime\cdot \left[N(T_A) - R\right] + \ibp{\left[N(T_A) - R\right]}{M} + \frac{R\beta}{M}
    \end{equation*}
    where one should recall that $M\triangleq \min\left(C_1\shs, k - R\right)$.
\end{restatable}

\begin{restatable}[Draining Phase, Continuing Integral Bound]{claim}{btwo}\label{clm:b2}
    One can bound the integral between consecutive separated visits by
    \begin{equation*}
        \ex{\int_{\visit{i}}^{\mintwo{\visit{i+1}}{X}}{[N(t) - R] \dd t}\middle| \filt{\visit{i}}} \leq \left[\frac{R}{M}\right]\cdot \ex{\mintwo{\visit{i+1}}{\cycle} - \visit{i} \middle | \vind \geq i} + \left[2 M +\frac{R}{M}\right] \left[v_i - v_{i-1} \right] + \ibp{M}{M}.
    \end{equation*}
\end{restatable}
\begin{restatable}[Draining Phase, Continuing Probability Bound]{claim}{bthree}\label{clm:b3}
    One can bound the probability that another visit occurs by
    \begin{equation*}
        \pr{\vind \geq i+1 \middle | \vind \geq i} \leq p_2,
    \end{equation*}
    where $p_2$ is a constant not depending on system parameters.
\end{restatable}

Before we move on to proving these claims, we first show to complete the proof of Lemma~\ref{lem:maintwo}, contingent on these three claims.
Applying Lemma~\ref{lem:waldstop}, we find that
\begin{align*}
    &\ex{\int_{T_A}^{X}{[N(t) - R] \dd t}\middle | \filt{T_A}} \\
    &\;\;\; \leq \left[ N(T_A) - R \right] \cdot \setuptime + \ibp{\ntar}{M} + \left[2M + 2\frac{R}{M}\right]\ex{X - T_A \middle| \filt{T_A}} +  \ibp{M}{M} \cdot \sum_{i=1}^{\infty}{p_2^{i-1}}\\
    &\;\;\; = \left[ N(T_A) - R \right] \cdot \setuptime + \ibp{\ntar}{M} + \left[2 M + 2 \frac{R}{M}\right]\ex{X - T_A \middle| \filt{T_A}} + \frac{1}{1- p_2} \ibp{M}{M};
\end{align*}
we take $A_4 \triangleq \frac{1}{1-p_2}$.

From here, to complete the proof, we only need to take the expectation of this quantity. We state this in claim form now, and defer the proof of this claim to Section~\ref{sec:taexpect}.
\begin{restatable}{claim}{taexpect}\label{clm:taexpect}
    Recall that $T_A \triangleq \minpar{t>0: Z(t) = R+1}$. Then,
\begin{align*}
    &\ex{ N(T_A) - R} \cdot \setuptime + \ex{\ibp{ \ntar}{M}}\\
    &\;\;\leq \left(B_5 \shs + B_6 \mu \beta \sqrt{R}\right)\cdot \beta + \ibp{B_5 \shs + B_6 \mu \beta \sqrt{R}}{M} + B_7\frac{\beta R}{M}.
\end{align*}
\end{restatable}
With this claim, we have shown Lemma~\ref{lem:maintwo}. \hfill \Halmos

All that remains now is to prove the claims outlined previously. 
\paragraph{Proof of Claim~\ref{clm:b3}.}
Before moving to the integral claims, we first observe that the probability in question is a down-crossing probability. In particular, if the $i$-th visit occurs, then the $(i+1)$-th visit will occur unless the renewal cycles end within the next $\setuptime$ time. In other words,
\begin{align*}
    \pr{\vind \geq i+1 \middle | \vind \geq i} = 1 - \pr{X < v_i + \setuptime \middle | \vind \geq i}.
\end{align*}
Now, note that the end of our renewal cycle $X$ is the moment the $(R+1)$-th server turns off. Since we are in the second phase of our cycle, this is simply the next time the number of jobs $N(t) \leq R$. Note also that, since we are in the second phase, $Z(t) \geq R$. Applying Claim~\ref{clm:dcprob}, we have that
\begin{equation*}
    \pr{X < v_i + \setuptime \middle | \vind \geq i} \geq 2\Phi\left( \frac{C_1}{\sqrt{2}} \right) - \frac{1}{100}.
\end{equation*}
Setting $C_1$ so that this final expression is equal to $p_2$, we again have our claim. \hfill \Halmos

\paragraph{The ``Wait-Then-Busy'' Period Idea.}
To prove the remaining integral claims, we make use of the following useful claim.
\begin{restatable}[Wait-Busy Period Bound]{claim}{waitbusy}\label{clm:waitbusy}
    Let $\tau$ be some stopping time. Let the next down-crossing $\dgen$, defined as
    \begin{equation*}
        \dgen \triangleq \minpar{t \geq 0: N(t + \tau) \leq R + M},
    \end{equation*}
    be the length of time until the number of jobs $N(t) \leq R + M$, where one should recall that $M\triangleq \min\left(C_1 \shs, k - R\right)$. Suppose that, at time $\tau$, we know that $Z(t + \tau) \geq R$ for any $t \in [0, \dgen]$. Then we have the following bound for the time integral of $N(t) - R$ from $\tau$ to $\tau + \dgen$:
    \begin{equation*}
        \ex{\int_{\tau}^{\dgen}{[N(t) - R] \dd t}\middle | \filt{\tau}} \leq \setuptime \cdot \left[ N\left(\tau \right) - (R+M) \right]^+ + \ibp{\left[N\left(\tau \right) - (R+M) \right]^+}{M} + \frac{R\beta}{M}.
    \end{equation*}
\end{restatable}
We defer the proof of Claim~\ref{clm:waitbusy} until Section~\ref{sec:waitbusy}. For now, we give a brief intuition for how the bound is derived and how we use it in our proof. Essentially, we can consider performing the following procedure at time $\tau$: First, watch the system for $\setuptime$ time. If the number of jobs ever dips below $R + M$ during this watching period, we can end our integral immediately. If the number of jobs $N(t)$ never dips below $R+M$ during this watching period, then we know for sure that we have at least $R + M$ servers on at time $\tau + \setuptime$, since the number of busy server $Z(t)$ satisfies
\begin{equation*}
    Z(t) = \min\left(k, \min_{s \in [t-\beta, t]}{N(s)}\right).
\end{equation*}
Moreover, by the same justification, those servers will \emph{stay} on until the number of jobs $N(t)$ dips below $R + M;$ in other words, they will stay on until time $\dgen$. The proof of the claim follows along essentially the same lines, formalizing things and performing computations using coupling and martingales.

\paragraph{Proof of Claim~\ref{clm:b1}.}
With Claim~\ref{clm:waitbusy} in hand, we return to proving the integral claims left over from our proof of Lemma~\ref{lem:maintwo}. To prove Claim~\ref{clm:b1}, we simply directly apply Claim~\ref{clm:waitbusy} with initial stopping time $\tau = T_A$ and with our specified down-crossing point $\dgen = v_1$. Doing this, we obtain
\begin{equation*}
        \ex{\int_{T_A}^{v_1}{[N(t) - R] \dd t}\middle | \filt{T_A}} \leq \setuptime \cdot \left[ N\left(T_A \right) - R \right]^+ + \ibp{\left[N\left(T_A \right) - R \right]^+}{M} + \frac{R \beta}{M},
\end{equation*}
which is precisely the claim. \hfill \Halmos

\paragraph{Proof of Claim~\ref{clm:b2}.}
To prove Claim~\ref{clm:b2}, we must go slightly further beyond the simple ``wait-then-busy'' period idea. The issue here is that the down-crossings we consider must be \emph{separated} by at least $\setuptime$ time; to get around this, we add in another waiting period. To be more specific, we imagine the following procedure for evaluating $\int_{v_i}^{\mintwo{v_{i+1}}{\cycle}}{\left[N(t) - R \right] \dd t}$: at time $v_i$, watch the system for a full setup time. If the number of jobs $N(t)$ dips down to $R$, then we have reached time $\cycle$ and we can stop integrating. On the other hand, if we haven't ended the renewal cycle yet, then we simply start another ''wait-then-busy'' period at time $\visit{i} + \setuptime$. Symbolically, we break down our integral in the following way:
\begin{equation}\label{eq:b2main}
    \int_{v_i}^{\mintwo{v_{i+1}}{\cycle}}{\left[N(t) - R \right] \dd t} = \int_{v_i}^{\mintwo{v_{i} + \setuptime}{\cycle}}{\left[N(t) - R \right] \dd t} + \left[\indc{X > v_i + \setuptime} \int_{v_i + \setuptime}^{\mintwo{v_{i+1}}{\cycle}}{\left[N(t) - R \right] \dd t} \right].
\end{equation}
With this decomposition it suffices to show that
\begin{equation}\label{eq:b2one}
    \ex{\int_{v_i}^{\mintwo{v_{i} + \setuptime}{\cycle}}{\left[N(t) - R \right] \dd t}\middle | \filt{v_i}} \leq M \left[ v_i - v_{i-1}\right]
\end{equation}
and
\begin{align}\label{eq:b2two}
    &\ex{\indc{X > v_i + \setuptime} \int_{v_i + \setuptime}^{\mintwo{v_{i+1}}{\cycle}}{\left[N(t) - R \right] \dd t} \middle | \filt{v_i}}\nonumber\\
    &\;\;\leq 
      \frac{R}{M} \ex{\mintwo{v_{i+1}}{X} - v_i\middle | \filt{v_i}} + \left[M+ \frac{R}{M}\right]\left[v_i - v_{i-1} \right] + \ibp{M}{M}.
\end{align}

To show \eqref{eq:b2one}, we note that, at time $v_i$, the end of the cycle $X$ is simply a down-crossing, and that, during the draining phase, the number of busy servers $Z(t) \geq R$. Applying Claim~\ref{clm:dcbnd}, we obtain
\begin{equation*}
    \ex{\int_{v_i}^{\mintwo{v_{i} + \setuptime}{\cycle}}{\left[N(t) - R \right] \dd t} \middle | \filt{v_i}} \leq [N(v_i) - R]\cdot \setuptime  = M \cdot \setuptime.
\end{equation*}
To finish our proof of \eqref{eq:b2one}, we must show that
\begin{equation*}
    \setuptime \leq \left[v_i - v_{i-1}\right].
\end{equation*}
This follows immediately from the fact that these are \emph{separated} visits; the next visit time $v_{i} > \beta + v_{i-1}$ by definition.

To show \eqref{eq:b2two}, we first apply the tower property then apply Claim~\ref{clm:waitbusy}, which gives
\begin{align*}
    &\ex{\indc{X > v_i + \setuptime} \int_{v_i + \setuptime}^{\mintwo{v_{i+1}}{\cycle}}{\left[N(t) - R \right] \dd t}\middle | \filt{v_i}}\\
    &\;\;= \ex{ \ex{\indc{X > v_i + \setuptime} \int_{v_i + \setuptime}^{\mintwo{v_{i+1}}{\cycle}}{\left[N(t) - R \right] \dd t}\middle | \filt{v_i + \setuptime}}\middle | \filt{v_i}} \\
    &\;\;= \ex{ \indc{X > v_i + \setuptime}\ex{ \int_{v_i + \setuptime}^{\mintwo{v_{i+1}}{\cycle}}{\left[N(t) - R \right] \dd t}\middle | \filt{v_i + \setuptime}}\middle | \filt{v_i}}\\
    &\;\;\leq \ex{ \indc{X > v_i + \setuptime}\left[\beta\cdot \left(N(v_i + \setuptime) - (R+M)\right)^+ + \ibp{\left[N\left(v_i + \setuptime\right) - (R+M)\right]^+}{M} + \frac{R\beta}{M}\right]\middle | \filt{v_i}}\\
     &\;\;\leq \ex{ \indc{X > v_i + \setuptime}\left[\beta\cdot \left(N(v_i + \setuptime) - (R)\right)^+ + \ibp{\left[N\left(v_i + \setuptime\right) - R\right]^+}{M} + \frac{R\beta}{M}\middle | \filt{v_i}\right]}.
\end{align*}

All that remains is to bound a number of conditional expectations. To proceed, we make use of the following claim:
\begin{restatable}{claim}{couplingEx}\label{clm:couplingEx}
     Given a stopping time $\tau$, let $\dgen \triangleq \minpar{t>0: N(t) \leq h}$ be the first time the number of jobs $N(t)$ crosses some threshold $h > N(\tau)$. Suppose we know that the number of busy servers $Z(t) \geq R - j$ for any time $t \in [\tau, \tau + \mintwo{\dgen}{\ell}]$, where the fixed time $\ell \in \filt{\tau}$. Then,
     \begin{equation}\label{eq:couplingfirst}
         \ex{\left[N\left(\tau + \ell\right) - h\right]\indc{\dgen > \ell}\middle | \filt{\tau}} \leq \mu j \ell + \left[N(\tau) - h\right]
     \end{equation}
     and
     \begin{equation}\label{eq:couplingsecond}
        \ex{\left[N\left(\tau + \ell\right) - h\right]^2\indc{\dgen > \ell}\middle | \filt{\tau}} \leq \left(\left[N(\tau) - h\right] + \mu j \ell\right)^2 + 2\mu R \ell.
     \end{equation}
\end{restatable}
For ease of reading, we defer the proof of this claim to Section~\ref{sec:couplingEx}.

\paragraph{Applying Claim~\ref{clm:couplingEx}.} We can apply Claim~\ref{clm:couplingEx} by noting that $\dgen = X- v_i$ is a hitting time, setting the initial time $\tau = v_i$, setting $\ell$ to be $\beta$, and noting that, for the rest of the renewal cycle, the number of busy servers $Z(t)\geq R$. Applying the claim, we see that the first term can be bounded by
\begin{equation*}
    \ex{ \indc{X > v_i + \setuptime}\left[\beta\cdot \left(N(v_i + \setuptime) - R\right)^+\right] \middle| \filt{v_i}} \leq \beta \left[N(v_i) - R\right] = \beta\cdot M \leq M \left[ v_i - v_{i-1}\right]
\end{equation*}
and the second term can be bounded by
\begin{align*}
     &\ex{ \indc{X > v_i + \setuptime} \ibp{\left[N\left(v_i + \setuptime\right) - R\right]}{M}  \middle | \filt{v_i}}\\
     &\;\;= \left[\frac{3}{2\mu M} + \frac{1}{\mu} + \frac{R}{\mu M^2} \right]\ex{\indc{X > v_i + \beta}\left( N(v_i + \beta) - R \right)\middle | \filt{v_i}}+ \left[\frac{1}{2 \mu M} \right] \ex{\indc{X > v_i + \beta} \left(N(v_i + \beta) - R\right)^2 \middle | \filt{v_i}}\\
     &\;\;= \left[\frac{3}{2\mu M} + \frac{1}{\mu} + \frac{R}{\mu M^2} \right]\left( N(v_i) - R\right) +  \left[\frac{1}{2 \mu M} \right] \left(N(v_i) - R\right)^2 + \frac{R \beta}{ M }\\
     &= \ibp{M}{M} + \frac{R}{M}\left[v_{i} - v_{i-1}\right].
\end{align*}
Via Markov's inequality, we see that the final term can be bounded by
\begin{equation*}
    \ex{\indc{X > v_i + \setuptime} \frac{R\beta}{M}\middle | \filt{v_i}} \leq \frac{R}{M} \ex{\mintwo{X}{v_{i+1}} - v_i \middle | \filt{v_i}},
\end{equation*}
which gives \eqref{eq:b2two}, and thus the claim.\hfill \Halmos


==> theorem1/lemma2_rev.tex <==
\newcommand{\visit}[1]{v_{#1}}
\newcommand{\threshtwo}{C_4 \shs}
\newcommand{\vind}{n_V}
\newcommand{\upb}[1]{\upsilon^{(\text{up})}_{#1}}
\newcommand{\downb}[1]{\upsilon^{(\text{down})}_{#1}}
\newcommand{\dnb}[1]{\downb{#1}}
\newcommand{\unb}[1]{\upb{#1}}
\newcommand{\mb}{M_B}
\newcommand{\tbind}{n_{b}}
\newcommand{\ntr}{\left[N(t) - R\right]}
\newcommand{\ibpfn}[3]{g\left(#1,#2,#3\right)}
% \newcommand{\systag}{\textup{sys}}
\newcommand{\donesys}{D^{\systag}_1 }
\newcommand{\upbnd}{\frac{b_2}{\sqrt{R}}}
\newcommand{\downbnd}{\frac{b_1 \sqrt{\beta}}{\sqrt{R}} + \frac{6}{R}}
\newcommand{\tbbnd}{\frac{1}{\mu}\left[\upbnd + \downbnd + \frac{1}{\mb}\right]  }
\newcommand{\ntk}{\left[ N\left(T_A\right) - k\right]}
\newcommand{\ntauk}{\left[ N\left(\tau\right) - k\right]}
\newcommand{\dgencouple}{\Tilde{\dgen}}
\newcommand{\downmod}{ b_1 \sqrt{\beta R}}

\subsection{Proof of Lemma~\ref{lem:maintwo}}\label{sub:maintwo}
We now prove our second main lemma, restated here for the reader's convenience.

\maintwo*

To prove this lemma, we again make use of Lemma~\ref{lem:waldstop}. 
We proceed through the usual two-step process, first defining the stopping time sequence we will analyze over, 
then proving the three preconditions of the lemma.

\begin{figure}
    \centering
    \includegraphics[scale=0.32,clip]{figures/sepvisits_new.pdf}
    \caption{A depiction of the separated visits defined in Section~\ref{sub:maintwo}. In this example, we find that the number of visits is $n_v = 4$. Notice that the second separated visit only happens when \emph{both} a setup time $\setuptime$ has passed \emph{and} the number of jobs $N(t)$ is currently $ \leq R+M$. For the third visit, these events happen simultaneously.}
    \label{fig:sepvisits}
\end{figure}

\paragraph{Definition of the upcrossings $\upb{i}$ and downcrossings $\downb{i}$.} 
Recall that the draining phase begins at time $T_A$. Let $\mb \triangleq \min\left(k-R, \max\left(\frac{\sqrt{R}}{D_1 \sqrt{\beta}}, 1 \right)\right)$ be a specially-set analysis threshold. Let the stopping time $\dnb{1} \triangleq \minpar{t \geq T_A: N(t) < R + \mb}$ be the first time the number of jobs $N(t)$ drops below $R +\mb$, and recursively define
\begin{equation*}
    \unb{i} \triangleq \minpar{ t\geq \dnb{i}: N(t) \geq R + \mb}
\end{equation*}
and 
\begin{equation*}
    \dnb{i+1} \triangleq \minpar{ t \geq \unb{i}: N(t) < R+ \mb}.
\end{equation*}

\paragraph{Application of Lemma~\ref{lem:waldstop}.}
Applying Lemma~\ref{lem:waldstop}, we take our initial stopping time to be $T_A$, our final stopping time to be $X$, our intervening stopping times to be $\dnb{i}$, our process of interest to be $\left[N(t) - R\right]$ and our counting index to be $\tbind$. Given that
\begin{equation}\label{eq:init_TB_int}
    \ex{\int_{T_A}^{\dnb{1}}{\ntr \dd t} \middle | \filt{T_A}} \leq        \left[N(T_A) - R\right]\cdot\left[\frac{1}{\mu} + \beta + \frac{1}{2\mu \mb} + \frac{R}{\mu \mb^2} \right] 
        + \left[N(T_A) - R\right]^2 \frac{1}{2 \mu \mb}
        + \frac{R \beta}{\mb^2},
\end{equation}
\begin{equation}\label{eq:succ_TB_int}
    \ex{\int_{\dnb{i}}^{\dnb{i+1}{\ntr \dd t}}\middle | \filt{\dnb{i}}} \leq \frac{1}{\mu} + \beta + \frac{1}{\mu \mb} \left[ 1 + \downmod + \frac{R}{\mb}\right]
        + \mb\cdot \left[\upbnd + \downbnd\right].
\end{equation}
and
\begin{equation}\label{eq:succ_TB_prob}
    \pr{\tbind \geq i+1 \middle | \tbind \geq i} \leq \frac{1}{\mb},
\end{equation}
we have 
\begin{align*}
    \ex{\int_{T_A}^{\dnb{1}}{\ntr \dd t}}  \leq  \ex{N(T_A) - R}\cdot\left[\frac{1}{\mu} + \beta + \frac{1}{2\mu \mb} + \frac{R}{\mu \mb^2} \right] 
        + \ex{\left(N(T_A) - R\right)^2} \frac{1}{2 \mu \mb}
        + \frac{R \beta}{\mb^2},
\end{align*}
and also that
\begin{align*}
    \ex{\int_{\dnb{1}}^{X}{\ntr \dd t}}\leq 
    \mb^2 \frac{1}{\mu}\left[\downbnd + \upbnd \right] 
    + \frac{\mb}{2 \mu} + \mb \beta 
    + \frac{1}{\mu}\left[ \frac{R}{\mb} + \frac{3}{2} \mb + \frac{1}{2} \right] 
    + \donesys \sqrt{\mu R \beta}.
\end{align*}

To finish off the proof, we use the following claim, whose proof we defer until Section~\ref{sec:taexpect}:
\begin{restatable}{claim}{taexpect}\label{clm:taexpect}
    Recall that $T_A \triangleq \minpar{t>0: Z(t) = R+1}$. Then,
\begin{align*}
    &\ex{ N(T_A) - R} \leq F_1 \mu \beta \sqrt{R}\left(1 + \frac{F_2}{\sqrt{\mu\beta}}\right)
\end{align*}
and
\begin{equation*}
    \ex{\left(N(T_A) - R\right)^2} \leq F_1^2 (\mu \beta)^2 R \left(1 + \frac{F_2}{\sqrt{\mu\beta}}\right)^2 + 2\mu \beta R,
\end{equation*}
where $F_1 = $ and $F_2 = $.
\end{restatable}

\paragraph{Proof of Lemma~\ref{lem:maintwo}.}
Applying Claim~\ref{clm:taexpect}, we find that
\begin{align*}
    \ex{\int_{T_A}^{\dnb{1}}{\ntr \dd t}}  &\leq  \ex{N(T_A) - R}\cdot\left[\frac{1}{\mu} + \beta + \frac{1}{2\mu \mb} + \frac{R}{\mu \mb^2} \right] 
        + \ex{\left(N(T_A) - R\right)^2} \frac{1}{2 \mu \mb}
        + \frac{R \beta}{\mb^2}\\
        % &\leq F_1 \mu \beta \sqrt{R}\left(1 + \frac{F_2}{\sqrt{\mu\beta}}\right)\left(1 + \frac{3}{2 \mu \beta}\right) +
\end{align*}


As such, to complete our proof it suffices to show \eqref{eq:init_TB_int},\eqref{eq:succ_TB_int},\eqref{eq:succ_TB_prob}, 

\paragraph{The ``Wait-Then-Busy'' Period Idea.}
To prove these inequalities, we make use of the following useful claim.
\begin{restatable}[Wait-Busy Period Bound]{claim}{waitbusy}\label{clm:waitbusy}
    Let $\tau$ be some stopping time. Let the next down-crossing $\dgen$, defined as
    \begin{equation*}
        \dgen \triangleq \minpar{t \geq 0: N(t + \tau) \leq R + h},
    \end{equation*}
    be the length of time until the number of jobs $N(t) \leq R + h$, where $h$ is some positive integer which is smaller than $k - R$. Suppose that, at time $\tau$, we know that $Z(t + \tau) \geq R$ for any $t \in [0, \dgen]$. Let $\dgencouple$ be the relative downcrossing time in a coupled system with exactly $R$ busy servers. Then we have the following bound for the time integral of $N(t) - R$ from $\tau$ to $\tau + \dgen$:
    \begin{align*}
        \ex{\int_{\tau}^{\tau + \dgen}{[N(t) - R] \dd t}\middle | \filt{\tau}} &\leq
        \left[N(\tau) - (R+h)\right]\cdot\left[\frac{1}{\mu} + \beta + \frac{1}{2\mu h} + \frac{R}{\mu h^2} \right]\\
        &\;\;+ \left(\left[N(\tau) - (R+h)\right]^+\right)^2 \frac{1}{2 \mu h} \\
        &\;\; + \ex{\mintwo{\beta}{\dgencouple}}\cdot\left[h + \frac{R}{h^2} \right]
    \end{align*}
\end{restatable}
We defer the proof of Claim~\ref{clm:waitbusy} until Section~\ref{sec:waitbusy}. For now, we give a brief intuition for how the bound is derived and how we use it in our proof. Essentially, we can consider performing the following procedure at time $\tau$: First, watch the system for $\setuptime$ time. If the number of jobs ever dips below $R + h$ during this watching period, we can end our integral immediately. If the number of jobs $N(t)$ never dips below $R+h$ during this watching period, then we know for sure that we have at least $R + h$ servers on at time $\tau + \setuptime$, since the number of busy server $Z(t)$ satisfies
\begin{equation*}
    Z(t) = \min\left(k, \min_{s \in [t-\beta, t]}{N(s)}\right).
\end{equation*}
Moreover, by the same justification, those servers will \emph{stay} on until the number of jobs $N(t)$ dips below $R + h;$ in other words, they will stay on until time $\dgen$. The proof of the claim follows along essentially the same lines, formalizing things and performing computations using coupling and martingales.

\subsubsection{Proof of \eqref{eq:init_TB_int}.}
To prove \eqref{eq:init_TB_int}, we simply apply Claim~\ref{clm:waitbusy} with starting time $\tau = T_A$ and threshold $h = \mb$. From there, we note $N(t) - (R+h) \leq N(t) - R$ and that $\ex{\mintwo{\beta}{\dnb{1}}} \leq \beta$; this gives the claim directly.

\subsubsection{Proof of \eqref{eq:succ_TB_int}.}
To prove \eqref{eq:succ_TB_int}, we break the integral into two parts; from the downcrossing $\dnb{i}$ to the upcrossing $\unb{i}$ and from the upcrossing $\unb{i}$ to the downcrossing $\dnb{i+1}$. 

First, we note that 
\begin{equation}
    \int_{\dnb{i}}^{\mintwo{\unb{i}}{X}}{\ntr \dd t} 
    \leq \left[\mintwo{\unb{i}}{X} - \dnb{i} \right]\cdot \mb,
\end{equation}
since $\unb{i}$ is the next time $N(t) \geq R + \mb$.
To bound $\ex{\mintwo{\unb{i}}{X} - \dnb{i}\middle | \filt{\dnb{i}}}$, we couple the system to an $M$/$M$/$\infty$ at time $\dnb{i}$, and note that the coupled up-crossing time $\Tilde{T_{(R+\mb-1)\to (R+\mb)}} + \dnb{i} \geq \unb{i} \geq \mintwo{\unb{i}}{X}$. From standard results on the $M$/$M$/$\infty$ (reproduced in Section~\ref{sec:downtodown} for completeness), we have that
\begin{equation*}
    \ex{\mintwo{\unb{i}}{X} - \dnb{i}\middle | \filt{\dnb{i}}} \leq \upbnd.
\end{equation*}

From $\unb{i}$ onwards, we use the ``wait-busy'' bound. Applying Claim~\ref{clm:waitbusy} with $h = \mb$, we obtain
\begin{align*}
    \ex{\int_{\unb{i}}^{\dnb{i+1}}{\ntr \dd t} \middle | \filt{\unb{i}}} &\leq \left[\frac{1}{\mu} + \beta + \frac{1}{2\mu \mb} + \frac{R}{\mu \mb^2} \right]
        + \frac{1}{2 \mu \mb}\\
        &\;\; + \ex{\mintwo{\beta}{\dnb{i+1} -\unb{i} }\middle | \filt{\unb{i}}}\cdot\left[\mb + \frac{R}{\mb} \right].
\end{align*}
To bound the conditional expectation of $\ex{\mintwo{\beta}{\dnb{i+1} - \unb{i}}\middle | \filt{\unb{i}}}$, it suffices to bound $\ex{\mintwo{\dgencouple}{\beta}}$, for the coupled relative downcrossing time $\dgencouple$. But note that $\dgencouple$ is exactly the busy period length of a critically-loaded M/M/1 queue with arrival rate and departure rate $k\lambda$. From standard results  (reproduced in Claim~\ref{clm:downint} for completeness), we have $\ex{\mintwo{\dgencouple}{\beta}}\leq \downbnd$ and thus that
\begin{equation*}
        \ex{\int_{\unb{i}}^{\dnb{i+1}}{\ntr \dd t} \middle | \filt{\unb{i}}} \leq \frac{1}{\mu} + \beta + \frac{1}{\mu \mb} \left[ 1 + \downmod + \frac{R}{\mb}\right]
        + \mb\cdot \left[\downbnd\right].
\end{equation*}


\subsubsection{Proof of \eqref{eq:succ_TB_prob}.}
To see \eqref{eq:succ_TB_prob}, we first note that, if there is another upcrossing, then there must be another downcrossing. As such, it suffices to upper bound $\pr{\unb{i} < X \middle | \dnb{i}}$. To do this, we note that the number of busy servers $Z(t) \geq R$. From Claim~\ref{clm:coupling}, it thus suffices to bound the corresponding probability in the coupled system with exactly $R$ busy servers. But this is simply the probability that, in a simple random walk started at $W(0) = \mb - 1$, the walk process $W(t)$ hits $W(t) = \mb$ before it hits $W(t) = 0$. Classically, this probability is $\frac{1}{\mb}$. \hfill \Halmos
 

==> theorem1/lemma3.tex <==
\newcommand{\longep}{\tau_L + \setuptime}
\newcommand{\xcouple}{\Tilde{X}}
\subsection{Proof of Lemma~\ref{lem:mainthree}.}
We now prove Lemma~\ref{lem:mainthree}, which we restate here.

\mainthree*

\paragraph{Preliminaries.}

The proof of this lemma is much simpler than the others. Before describing our strategy, we first state some preliminaries. Recall from Section~\ref{sec:lemma1} the definition of the start of the $j$-th epoch, $\tau_j$:
\begin{equation*}
    \tau_j \triangleq \minpar{t\geq 0: N(t) \leq R - j}.
\end{equation*}
We call the period $\bigg[\tau_j, \mintwo{\tau_{j+1}}{T_A} \bigg )$ the $j$-th epoch, and say epoch $j$ occurs if $\tau_j < T_A$. Say an epoch $j$ is long if it lasts longer than a setup time $\setuptime$; note that such an epoch must exist, since servers can only turn on during long epochs, and a server must turn on before the accumulation phase is over. Let $L$ be the index of the \emph{first} long epoch, i.e.
\begin{equation*}
    L \triangleq \minpar{ j \in  \left \{ 0,1,2,\dots, R\right\}: \mintwo{\tau_{j+1}}{T_A} - \tau_j > \beta}.
\end{equation*}
Note that, although the random time $\tau_L$ is \emph{not} a stopping time (we do not know how long an epoch will last when the epoch starts), the first moment we can identify epoch $L$, the random time $\tau_L + \setuptime$, \emph{is} a stopping time. Moreover, we know that $\tau_L +\setuptime < T_A$. From here, one sees that
\begin{align*}
    \ex{X} &= \ex{\longep } + \ex{X - \left(\longep\right)}\\
    & \geq \setuptime + \ex{X - \left(\longep\right)}.
\end{align*}
To complete the proof, we show two claims. First, we show via a simple coupling argument that
\begin{equation}\label{eq:mainthree1}
    \ex{X - \left(\longep\right)}\geq \bp{\ex{N\left(\longep\right)- R}}{k-R},
\end{equation}
then, via martingale arguments, we show that
\begin{equation}\label{eq:mainthree2}
    \ex{N\left(\longep\right)- R} \leq \mu \beta \ex{L}.
\end{equation}
Combining the above with Claim~\ref{clm:lbound}, which states
\begin{equation}\label{eq:mainthree3}
    \ex{L} \geq D_1 \sqrt{R},
\end{equation}
we obtain the result.

\paragraph{Proof of \eqref{eq:mainthree1}.}
To show \eqref{eq:mainthree1}, we make a simple coupling argument. Consider a coupled system with the same arrival process but the maximum possible departure rate, $k\mu$. In other words, define for all time $t\geq \longep$
\begin{equation*}
    \ncouple(t) \triangleq N \left(\longep\right) + A\left( (\longep, t]\right) - \depOp{k}{(\longep, t]}.
\end{equation*}
Since $Z(t) \leq k$, it follows that $N(t) \leq \ncouple(t)$ for all $t \geq \longep$. Naturally then, the coupled down-crossing time $\xcouple \triangleq \minpar{t \geq \longep: \ncouple(t) \leq R}$ must be smaller than the end of our renewal cycle, since the cycle ends once a similar down-crossing occurs \emph{after} the $(R+1)$-th server has turned on, i.e.
\begin{equation*}
    X \triangleq \minpar{t>0: Z(t^-) = R+1, Z(t) = R} = \minpar{t> T_A: N(t) \leq R}.
\end{equation*}
Thus we have
\begin{align*}
    \ex{X - \left(\longep\right)\middle | \filt{\longep}} 
    &\geq \ex{\xcouple - \left(  \longep \right)\middle | \filt{\longep}}\\
    &= \bp{\left[N\left(\longep\right)- R\right]^+}{k-R}\\
    &\geq \bp{N\left(\longep\right)- R}{k-R}.
\end{align*}
Since the length of a busy period scales linearly with the number of jobs which start it, we have \eqref{eq:mainthree1} via linearity of expectation.

\paragraph{Proof of \eqref{eq:mainthree2}.}
To bound $\ex{N\left(\longep\right)}$, we make an extended martingale argument.
First, by conditioning on the value of the index $L$, it's clear that
\begin{equation*}
    \ex{N\left(\longep\right)} = \sum_{j=0}^{R}{\ex{N\left(\longep\right)\indc{L = j}}}.
\end{equation*}
Taking one of these terms, we also have that
\begin{align}
    \ex{N\left(\longep\right)\indc{L = j}} &=  \ex{N\left(\longep\right)\indc{L = j}\indc{L \geq j}}\nonumber\\
    &= \ex{\ex{N\left(\longep\right)\indc{L = j} \indc{L \geq j}\middle | \filt{\tau_j}}} \label{eq:mt2i1}\\
    &= \ex{\indc{L \geq j}\ex{N\left(\longep\right)\indc{L = j} \middle | \filt{\tau_j}}}\label{eq:mt2i2}\\
    &= \ex{\indc{L \geq j}\ex{N\left(\tau_j + \setuptime\right)\indc{L = j} \middle | \filt{\tau_j}}}\label{eq:mt2i3},
\end{align}
where \eqref{eq:mt2i1} is an application of the tower property, and \eqref{eq:mt2i2} follows from the fact that we learn that $L \geq j$ only at time $\tau_j$ (if time $\tau_j$ does not occur, then $L < j$).

\paragraph{Simplification of \eqref{eq:mt2i3}.}
We now simplify the expectation term from \eqref{eq:mt2i3}. We do this in two steps, first rewriting the event $\brc{L=j}$ as an event concerning a particular down-crossing, and, second, rewriting the value of $N\left(\longep\right)$ as the value of a particular martingale. 

First, we rewrite the event $\brc{L=j}$. Note that, with certainty, we know the state at time $\tau_j$: since epoch $j$ has just begun, there are no servers in setup and $N(\tau_j) = Z(\tau_j) = R - j$. Assuming that the system has made it to time $\tau_j$ without having a long epoch, i.e. the indicator $\indc{L \geq j} = 1$, then the event $\brc{L = j}$ is simply the probability that, for the next $\setuptime$ time, the number of jobs $N(t)$ does not dip down to $R - (j+1)$. In other words, if we define $\gamma$ as $\tau_{j+1} - \tau_j$, or equivalently as
\begin{equation*}
    \gamma \triangleq \minpar{ t > 0: N(\tau_j + t) \leq R - (j+1)},
\end{equation*}
then we can rewrite the event $\brc{L = j}$ as $\brc{L = j} = \brc{ \gamma \geq \setuptime}$. With this, we find that
\begin{equation*}
    \indc{L \geq j}\ex{N\left(\tau_j + \setuptime\right)\indc{L = j} \middle | \filt{\tau_j}} = \indc{L \geq j}\ex{N\left(\tau_j + \setuptime\right)\indc{\gamma \geq \setuptime} \middle | \filt{\tau_j}};
\end{equation*}
note that this new event \emph{does not} depend on what happened before time $\tau_j$.

Second, we note that, from time $\tau_j$ until either time $\tau_j + \setuptime$ or time $\tau_j + \gamma$, we can very succinctly describe the sample-path behavior of $N(t)$. In particular, we know that the number of busy servers $Z(t) = R -j$ during this interval, and thus that
\begin{equation*}
    N(\tau_j + t) = R - j + A(\tau_j,\tau_j + t) - \depOp{R - j}{(\tau_j,  \tau_j + t]},
\end{equation*}
for any $t \in \left[0, \mintwo{\gamma}{\setuptime}\right]$.
Since the function $N(\tau_j + t)$ is the difference between two independent Poisson processes over this interval, it follows that the function
\begin{equation*}
    V(t) = \ncouple(\tau_j + t) - \mu j t
\end{equation*}
is a martingale over this interval. Thus, we have that
\begin{align*}
    \ex{N\left(\tau_j + \setuptime\right)\indc{\gamma \geq \setuptime} \middle | \filt{\tau_j}} &= \ex{\left[V\left(\setuptime\right) + \mu j \beta\right]\indc{\gamma \geq \setuptime} \middle | \filt{\tau_j}}\\
    &= \ex{V\left(\setuptime\right)\indc{\gamma \geq \setuptime} \middle | \filt{\tau_j}} + \mu j \setuptime \pr{\gamma \geq \setuptime \middle | \filt{\tau_j}}.
\end{align*}
Noting that $\setuptime = \mintwo{\setuptime}{\gamma}$ if $\gamma \geq \setuptime$, that the martingales initial value $V(0) = R - j$, and that its down-crossing value $V(\gamma) = R - (j+1)$, we find
\begin{align*}
    V\left(\setuptime\right)\indc{\gamma \geq \setuptime} &= V\left(\mintwo{\gamma}{\setuptime}\right)\indc{\gamma \geq \setuptime}\\
    &= V\left(\mintwo{\gamma}{\setuptime}\right) - V\left(\mintwo{\gamma}{\setuptime}\right)\indc{\gamma < \setuptime}\\
    &= V\left(\mintwo{\gamma}{\setuptime}\right) - \left[R - (j+1)\right]\indc{\gamma < \setuptime}.
\end{align*}
Applying Doob's Optional Stopping Theorem, we obtain that
\begin{align*}
    \ex{V(\setuptime) \indc{\gamma \geq \setuptime}\middle | \filt{\tau_j}} &= \ex{V\left(\mintwo{\gamma}{\setuptime}\right)\middle | \filt{\tau_j}} - \left(R - j - 1\right) \pr{\gamma < \beta \middle | \filt{\tau_j}}\\
    &= R - j - \left(R - j - 1\right) \pr{\gamma < \beta \middle | \filt{\tau_j}}\\
    &= \left(R - j \right)\pr{\gamma \geq \beta \middle | \filt{\tau_j}} + \pr{\gamma < \beta \middle | \filt{\tau_j}}.
\end{align*}
Thus, we find that
\begin{align*}
    \ex{N\left(\tau_j + \setuptime\right)\indc{\gamma \geq \setuptime} \middle | \filt{\tau_j}} = \left(R - j \right)\pr{\gamma \geq \beta \middle | \filt{\tau_j}} + \pr{\gamma < \beta \middle | \filt{\tau_j}} + \mu j \beta \pr{\gamma \geq \beta \middle | \filt{\tau_j}}
\end{align*}
and thus that
\begin{align*}
    \indc{L \geq j} \ex{N\left(\tau_j + \setuptime\right)\indc{\gamma \geq \setuptime} \middle | \filt{\tau_j}} &= \indc{L \geq j} \left[(R-j + \mu \setuptime j)\pr{L = j \middle | \filt{\tau_j}} + \pr{L \geq j + 1 \middle | \filt{\tau_j}}\right]\\
    &= (R - j + \mu \beta j) \pr{L = j \middle | \filt{\tau_j}} + \pr{L \geq j +1 \middle | \filt{\tau_j}}.
\end{align*}
Returning to \eqref{eq:mt2i3}, we find that
\begin{align*}
    \ex{N\left(\longep\right)\indc{L = j}} &= \left(R - j + \mu \setuptime j\right) \pr{L = j} + \pr{L \geq j + 1},
\end{align*}
and thus that
\begin{align*}
    \ex{N(\left(\longep \right)} &= R + (\mu \setuptime - 1) \sum_{j=0}^{R}{j \pr{ L = j}} + \sum_{j=0}^{R}{\pr{L \geq j}}\\
    &= R + \left(\mu\setuptime - 1\right) \ex{L} + \ex{L}\\
    &= R + \mu\setuptime \ex{L},
\end{align*}
as desired. 

\paragraph{Proof of \eqref{eq:mainthree3}.} To complete the proof, we need only show
\eqref{eq:mainthree3}. Following the lines of \cite{WHW}, we show
\begin{restatable}{claim}{lbound}\label{clm:lbound}
    Let $L$ be the first \emph{long} epoch, i.e. let $L \triangleq \minpar{j \in N: \tau_{j+1} - \tau_j > \setuptime}$. Then,
    \begin{equation*}
        \ex{L} \geq \frac{2}{3}\sqrt{\frac{\pi}{2}} \sqrt{R},
    \end{equation*}
    where $\frac{2}{3}\sqrt{\frac{\pi}{2}} \geq 0.83$.
\end{restatable}

We defer the proof of this claim to Section~\ref{sec:lbound}. \hfill \Halmos





==> theorem2/lemma_LB_int.tex <==

We prove this lemma in the same way as \cite{WHW}; the proof is replicated here for completeness. Recall the definition of the beginning of epoch $i$, i.e.
$\tau_i \triangleq \minpar{t > 0: N(t) \leq R - i}$; note that epoch $i$ ends when either epoch $i+1$ starts (at time $\tau_{i+1}$) or when the $(R+1)$-th server turns on (at time $T_A$). Recall also, from Section~\ref{sec:cycle_lb}, the definition of $L \triangleq \minpar{i \geq \mathbb{N}: \tau_{i+1} - \tau_{i} \geq \beta}$, the index of the first \emph{long} epoch.
Note that $\tau_L + \beta \leq T_A$, since an epoch must be long if \emph{any} servers turn on during the epoch.

To analyze the integral in question, we split it up based on time $\tau_L  + \beta$. That is, we first note that
\begin{equation*}
    \ex{\int_0^{X}{Q(t) \dd t}} 
    = \ex{\int_0^{\tau_L + \setuptime}{Q(t) \dd t}} + \ex{\int_{\tau_L+ \setuptime}^{X}{Q(t) \dd t}},
\end{equation*}
then show that
\begin{equation}\label{eq:int_taul}
    \ex{\int_0^{\tau_L + \setuptime}{Q(t) \dd t}} \geq \mu \ex{L} \frac{\beta^2}{2}
\end{equation}
and
\begin{equation}\label{eq:int_aft}
    \ex{\int_{\tau_L+ \setuptime}^{X}{Q(t) \dd t}} \geq \ibp{\left[ \ex{N(\tau_L + \beta)} - k\right]^+}{k-R}.
\end{equation}

From there, we can apply \eqref{eq:mainthree3} and Claim~\ref{clm:lbound}, which show, respectively, that
\begin{equation*}
    \ex{N\left(\tau_L + \beta\right)} \geq R + \mu \beta \ex{L}.
\end{equation*}
and
\begin{equation*}
    \ex{L} \geq \frac{2}{3}\sqrt{\frac{\pi}{2}} \sqrt{R}.
\end{equation*} 

It thus suffices to show \eqref{eq:int_taul} and \eqref{eq:int_aft}.


\subsubsection{Proof of \eqref{eq:int_taul}.}
To show \eqref{int_tau}, we first condition on whether $L \geq i$, giving
\begin{align*}
    \ex{\int_0^{\tlba}{Q(t) \dd t}} &= \sum_{i=0}^{\infty}{\ex{\int_{\tau_i}^{\mintwo{\tau_i + \beta}{\tau_{i+1}}}
    {Q(t) \dd t}\indc{L \geq i}}}\\
    &=  \sum_{i=0}^{\infty}{\ex{\int_{\tau_i}^{\mintwo{\tau_i + \beta}{\tau_{i+1}}}
    {Q(t) \dd t}\middle | \filt{\tau_i}}\pr{L \geq i}}.
\end{align*}

To further develop this conditional expectation, we note that during the interval $[\tau_i, \mintwo{\tau_i + \beta}{\tau_{i+1}})$, the system must have exactly $Z(t) = R -i$ busy servers running, meaning that $Q(t) = N(t) - (R - i)$. 
Defining a coupled process $\qcouple(t)$ as 
\begin{equation*}
    \qcouple(t) =  A(\tau_i, t) - \depOp{R-i}{\tau_i, t},
\end{equation*}
we see that $Q(t)$ and $\qcouple(t)$ coincide during the interval in question. Moreover, one can redefine the stopping time $\gamma = \tau_{i+1}$ as $\minpar{t>\tau_i: \qcouple(t) = -1}$. Noting that $Q\left( \mintwo{\gamma}{t}\right) = -1$ for any time $t > \gamma$, we find that
\begin{align*}
    \int_{\tau_i}^{\mtb}{Q(t) \dd t} &= \int_{\tau_i}^{\mtb}{\qcouple(t) \dd t}\\
    &= \int_{\tau_i}^{\mtb}{\qcouple\left(\mintwo{t}{\tau_{i+1}}\right) \dd t} +  \int_{\mtb}^{\tau_i + \beta}{\left(\qcouple\left(\mintwo{t}{\tau_{i+1}}\right) + 1\right) \dd t} \\
    &=\int_{\tau_i}^{\tau_i + \beta}{\qcouple\left(\mintwo{t}{\tau_{i+1}}\right) \dd t} + \left[ \beta - \mintwo{\beta}{\tau_{i+1} - \tau_i}\right]\\
    &\geq \int_{\tau_i}^{\tau_i + \beta}{\qcouple\left(\mintwo{t}{\tau_{i+1}}\right) \dd t}.
\end{align*}
Taking the conditional expectation at time $\tau_i$, we find
\begin{align*}
    \ex{\int_{\tau_i}^{\tau_i + \beta}{\qcouple\left(\mintwo{t}{\tau_{i+1}}\right) \dd t}\middle | \filt{\tau_i}} = \int_{\tau_i}^{\tau_i + \beta}{\ex{\qcouple\left(\mintwo{t}{\tau_{i+1}}\right)\middle | \filt{\tau_i}} \dd t}.
\end{align*}
Noting that $V_L(t) = \qcouple(t) - \mu i \left[t - \tau_i\right]$ is a martingale, and that $\mintwo{t}{\tau_{i+1}}$ is an almost-surely bounded stopping time, we have that
\begin{align*}
    \qcouple(\tau_i) &= V_L(\tau_i) = 0\\
                    &= \ex{V_L\left(\mintwo{t}{\tau_{i+1}}\right)\middle| \tau_i}\\
                    &= \ex{\qcouple\left(\mintwo{t}{\tau_{i+1}}\right)\middle| \filt{\tau_i}} - \mu i \ex{\mintwo{t}{\tau_{i+1}}\middle| \filt{\tau_i}}.
\end{align*}
Since 
\begin{equation*}
    \ex{\mintwo{t}{\tau_{i+1}}\middle|\filt{\tau_i}} \geq t\cdot \pr{\tau_{i+1} - \tau_i \geq t} \geq t \cdot \pr{\tau_{i+1} - \tau_i \geq t} = t \pr{L = i \middle | L \geq i},
\end{equation*}
we have 
\begin{align*}
   \pr{L\geq i} \ex{\int_{\tau_i}^{\mtb}{Q(t) \dd t}\middle| L \geq i}  &\geq \pr{L \geq i} \ex{\int_{\tau_i}^{\tau_i + \beta}{\qcouple\left(\mintwo{t}{\tau_{i+1}}\right) \dd t}\middle | L \geq i}\\
    & \geq \int_{\tau_i}^{\tau_i + \beta}{\mu i t \pr{L = i}}\\
    &= \mu \frac{\beta^2}{2} i \pr{L=i}
\end{align*}
Summing across all $i$, we obtain \eqref{eq:int_taul}.

\subsubsection{Proof of \eqref{eq:int_aft}.}
To prove \eqref{eq:int_aft}, we make a simple coupling argument. Let $\eta_k \triangleq \minpar{t\geq \tau_L + \beta: N(t) \leq k}$. Since the draining phase starts at $T_A \geq \tau_L + \beta$ and the end of the cycle $X = \minpar{t \geq T_A: N(t) \leq R}$, we know that $X \geq \eta_k$. Moreover, we know the number of busy servers $Z(t) \leq k$; it follows by Claim~\ref{clm:coupling} that we can define $\ncouple(t)$ as 
\begin{equation*}
    \ncouple(t) \triangleq N\left(\tau_L + \beta\right) + A\left(\tau_L + \beta, t\right) - \depOp{k}{\left(\tau_L + \beta, t\right)}
\end{equation*}
and have $\ncouple(t) \leq N(t)$ for any $t > \tlba.$ Even further, we can defined a coupled hitting time $\Tilde{\eta}_k \triangleq \minpar{t > \tlba: \ncouple(t) \leq k}$ which must happen before $\eta_k$. In other words,
\begin{align*}
    \int_{\tlba}^{X}{Q(t) \dd t} &\geq \int_{\tlba}^{\eta_k}{Q(t) \dd t}\\
    &\geq \int_{\tlba}^{\eta_k}{\left[N(t) - k\right] \dd t}\\
    &\geq \int_{\tlba}^{\Tilde{\eta}_k}{\left[\ncouple(t) - k\right] \dd t}.
\end{align*}
This final term is just the time integral of the number of jobs in system over a M/M/1 busy period started by $\left[N\left(\tlba\right) - k\right]^+$ jobs, where jobs arrive at rate $k\lambda$ and depart at rate $k\mu$. 
Accordingly, we have
\begin{align*}
     \ex{\int_{\tlba}^{X}{Q(t) \dd t}} 
     &\geq \ex{\ibp{\left[N\left(\tlba\right) - k \right]^+}{k - R}}\\
     &\geq \ibp{\ex{N\left(\tlba\right) - k }^+}{k-R}\\
     &\geq \ibp{\ex{\left[N\left(\tlba\right) - R - \left( k - R\right)\right]^+}}{k-R},
\end{align*}
where in the last two lines we have applied Jensen's inequality.\hfill  \Halmos

==> theorem2/lemma_UB_TA.tex <==
\paragraph{Defining a coupling.} To prove Lemma~\ref{lem:ubacc_cycle}, we first note that, during the accumulation phase, we have two bounds on the number of busy servers $Z(t)$: it must be less than the total number of jobs $N(t)$ and it must be less than $R$; the former because every busy server must be working on a job, and the latter because otherwise the accumulation phase would be over. Thus, we can define a coupled $M/M/R$ system for which the number of jobs $\ncac(t)$ in the coupled system is always at least the number of jobs $N(t)$ in the original system.

\paragraph{How we use the coupling.} To use this coupled process to bound $\ex{T_A}$, recall that the accumulation point $T_A$ is the first time the $(R+1)$-th server turns on. Accordingly, one can also think of this as the first time that there has been at least $R+1$ jobs in the system for $\beta$ time.  Thus, if we define a coupled accumulation point
$\tac \triangleq \minpar{t \geq \beta : \min_{s \in [t-\beta, t)}{\ncac(t)} \geq R+1}$, then we know $\tac \geq T_A$. In other words, it suffices to bound $\ex{\tac}$.

\paragraph{Applying Lemma~\ref{lem:waldstop}.} 
We bound $\ex{\tac}$ using the intervening method of Lemma~\ref{lem:waldstop}. As such, we define a few stopping times, then list the preconditions/claims that we will satisfy to complete the proof of Lemma~\ref{lem:ubacc_cycle}.

\paragraph{Definition of $\upc$ and $\dnc$.} Let the initial cycle-downcrossing occur at $\dnc_0 \triangleq  0$ and iteratively define the up-crossings $\upc$ and down-crossings $\dnc$ as
\begin{equation*}
    \upc_{i} \triangleq \minpar{t\geq \dnc_i: \ncac(t) \geq R+1} 
\end{equation*}
and 
\begin{equation*}
    \dnc_{i+1} \triangleq \minpar{t \geq \upc_{i}: \ncac(t) \geq R+1}.
\end{equation*}

\paragraph{Application of Lemma~\ref{lem:waldstop}.}
Applying Lemma~\ref{lem:waldstop} using $0= \dnc_0$ as our starting point, the coupled accumulation point $\tac$ as our ending point, our test function as $Y_t =1$, and the cycle-upcrossings $\left(\dnc_i\right)$ as our intervening stopping times, we now must prove that
\begin{equation}\label{eq:acc_init}
    \ex{\upc_{i} - \dnc_i \middle | \cind \geq i } \leq \frac{1}{\mu} e^{\frac{1}{12 R}} \sqrt{1 + \frac{1}{R}} \frac{\sqrt{2 \pi}}{\sqrt{R}} \leq \frac{c_3}{\mu \sqrt{R}},
\end{equation}
\begin{equation}\label{eq:acc_succ}
    \ex{\mintwo{\tac}{\dnc_{i+1}} - \upc_{i} \middle| \cind \geq i} \leq b_1\sqrt{\frac{\beta}{\mu R}} + \frac{6}{\mu R},
\end{equation}
and
\begin{equation}\label{eq:acc_prob}
    \pr{ \cind \geq i+1 \middle | \cind \geq i} \leq 1 -  \frac{b_1}{\sqrt{2}} e^{-\frac{1}{3(\mu 2 R \beta-1)}} \frac{1}{\sqrt{\mu 2 R \beta + 2}} \leq 1 - \frac{b_1 c_4}{\sqrt{\mu R \beta}},
\end{equation}
where $b_1 \triangleq \sqrt{\frac{2}{\pi}}$, $c_3 = 1.001\sqrt{2 \pi }$, and $c_4 = 0.499$

\paragraph{Completion of Proof, assuming \eqref{eq:acc_init}, \eqref{eq:acc_succ}, and \eqref{eq:acc_prob}.}
Applying Lemma~\ref{lem:waldstop}, one finds that
\begin{align*}
    \ex{\tac} &= \sum_{i=0}^{\infty}{\ex{\mintwo{\tac}{\dnc_{i+1}} - \dnc_i \middle | \cind \geq i} \pr{\cind \geq i}}\\
    &\leq \left[\frac{c_3}{\mu \sqrt{R}} + \frac{b_1 \sqrt{\beta}}{\sqrt{\mu R}} + \frac{6}{\mu R} \right] \frac{\sqrt{\mu R \beta}}{b_1 c_4}\\
    &= \frac{1}{\mu}\left[\frac{c_3}{b_1 c_4}\sqrt{\beta} + \frac{1}{c_4} \right]
\end{align*}

\subsubsection{Proof of \eqref{eq:acc_init}.}
To prove \eqref{eq:acc_init}, we note that, since our coupled system is an $M/M/R$, the expected time $\ex{\upc_{i} - \dnc_i \middle | \cind \geq i }$ is simply the expected passage time from state $R$ to $R+1$ in an $M$/$M$/$R$ ( and equivalently an $M$/$M$/$R$/$R+1$, an $M$/$M$/$R$ which can contain only $R+1$ jobs. Solving, one finds that 
\begin{align*}
    \ex{T_{R\to(R+1)}} &\leq \ex{T_{(R+1)\to(R+1)}}\\
    &=\frac{1}{\mu(R+1)} \frac{1}{\pi_{R+1}}\\
    &= \frac{1}{\mu(R+1)} \frac{\sum_{i=0}^{R+1}{\frac{R^i}{i!}}}{\frac{R^{R+1}}{(R+1)!}}\\
    &\leq \frac{1}{\mu (R+1)} e^{R}\frac{(R+1)!}{R^{R+1}}\\
    &\leq \frac{1}{\mu (R+1)} e^{R}\frac{e^{\frac{1}{12 (R+1}}\sqrt{2 \pi (R+1)}(R+1)^{R+1} e^{-(R+1)}}{R^{R+1}}\\
    &= e^{\frac{1}{12 R}}\frac{1}{\mu} \sqrt{2 \pi} \frac{\sqrt{R+1}}{R} \left(1 + \frac{1}{R}\right)^R e^{-1}\\
    &\leq \frac{1}{\mu} e^{\frac{1}{12 R}} \sqrt{1 + \frac{1}{R}} \frac{\sqrt{2 \pi}}{\sqrt{R}}\\
    &\leq \frac{1}{\mu} 1.006 \frac{\sqrt{2 \pi}}{\sqrt{R}}\\
    &\triangleq \frac{c_3}{\mu \sqrt{R}}
\end{align*}

\subsubsection{Proof of \eqref{eq:acc_succ}.}
To bound the expected time $\ex{\mintwo{\tac}{\dnc_{i+1}} - \upc_i \middle | \cind \geq i}$, we first note that, if $\upc_i + \beta \leq \dnc_{i+1}$, then $\tac = \upc_i + \beta$. Likewise, if $\upc_i + \beta > \dnc_{i+1}$, then $\tac > \dnc_{i+1}$. It follows that, given that $\cind \geq i$, the time $\mintwo{\tac}{\dnc_{i+1}} = \mintwo{\beta + \upc_i}{\dnc_{i+1}}$. Thus, we have that
\begin{equation*}
    \ex{\mintwo{\tac}{\dnc_{i+1}} - \upc_i \middle | \cind \geq i} = \ex{\mintwo{\beta}{\dnc_{i+1} - \upc_i} \middle | \cind \geq i} = \int_0^{\beta}{\pr{\dnc_{i+1} - \upc_i > s\middle| \cind \geq i} \dd s}.
\end{equation*}

We continue by bounding this tail probability. To begin, note that, while $\ncouple(t)$ stays above $R+1$, the dynamics of $\ncouple$ are precisely that of a critically-loaded $M$/$M$/$1$ queue with arrival rate and departure rate equal to $k\lambda$. The tail probability we are interested in bounding is precisely the probability that a busy period (started with 1 job) in such a system lasts longer than $s$ time. Applying Claim~\ref{clm:contdown}, one finds that, for any $t \geq \frac{3}{\mu 2 R}$,
\begin{equation*}
    \pr{\dnc_{i+1} - \upc_i > s\middle| \cind \geq i} \leq b_1 \left( \frac{1}{\sqrt{\mu 2 R s}} + \frac{b_2}{(\mu 2 R s)^{3/2}}\right).
\end{equation*}
Integrating, we find that
\begin{align*}
    \int_0^{\beta}{\pr{\dnc_{i+1} - \upc_i > s\middle| \cind \geq i} \dd s} &\leq \frac{3}{\mu 2 R} + \frac{b_1}{\sqrt{2}} \int_{\frac{3}{\mu 2 R}}^{\beta} {\frac{1}{\sqrt{\mu 2 R s}} + \frac{b_2}{(\mu 2 R s)^{3/2}} \dd s}\\
    &\leq \frac{3}{\mu 2 R} + \frac{b_1}{\sqrt{2}} \left[\sqrt{\frac{2 \beta}{ \mu R}} + b_2 \sqrt{\frac{2}{3}}  \frac{1}{\mu R} \right]\\
    &= b_1  \sqrt{\frac{\beta}{\mu R}} + \left( \frac{3}{2} + (b_1 + 2.5) \sqrt{\frac{2}{3}}\right)\frac{1}{\mu R}\\
    &\leq \frac{2}{\sqrt{\pi}}\sqrt{\frac{\beta}{\mu R}} + \frac{6}{\mu R}.
\end{align*}
\hfill \Halmos

\subsubsection{Proof of \eqref{eq:acc_prob}.}
To prove \eqref{eq:acc_prob}, it suffices to note that, upon conditioning on the filtration at $\upc_i$, the probability $\pr{ \cind \geq i+1 \middle | \cind \geq i}$
is simply the probability that a busy period in a critically-loaded M/M/1, with arrival and departure rate equal to $\mu R$, ends before $\beta$ time has passed. Applying Claim~\ref{clm:contdown}, one finds that this is
\begin{equation*}
    \pr{ \cind \geq i+1 \middle | \cind \geq i} \geq 1 -  \frac{b_1}{\sqrt{2}} e^{-\frac{1}{3(\mu 2 R \beta-1)}} \frac{1}{\sqrt{\mu 2 R \beta + 2}}. \hfill \Halmos
\end{equation*}

==> theorem2/lemma_UB_TB.tex <==
\newcommand{\bind}{n_\zeta}
\newcommand{\dnb}[1]{\zeta_{#1}^{(\textup{d})}}
\newcommand{\unb}[1]{\zeta_{#1}^{(\textup{u})}}
\newcommand{\tbthresh}{M_L}

We now prove the upper bound on $\ex{X - T_A}$. We make use of the ``wait-busy'' idea from Section~\ref{sec:waitbusy} as well as our main tool, Lemma~\ref{lem:waldstop}. As such, we begin by defining some stopping times.

\paragraph{Definition of $\dnb{i}$ and $\unb{i}$. }
Recall that the draining phase begins at time $T_A$. Let $\tbthresh \triangleq \min\left(k-R, \max\left(\frac{\sqrt{R}}{D_1 \sqrt{\beta}}, 1 \right)\right)$ be a specially-set analysis threshold. Let the stopping time $\dnb{1} \triangleq \minpar{t \geq T_A: N(t) < R + \tbthresh}$ be the first time the number of jobs $N(t)$ drops below $R +\tbthresh$, and recursively define
\begin{equation*}
    \unb{i} \triangleq \minpar{ t\geq \dnb{i}: N(t) \geq R + \tbthresh}
\end{equation*}
and 
\begin{equation*}
    \dnb{i+1} \triangleq \minpar{ t \geq \unb{i}: N(t) < R+ \tbthresh}.
\end{equation*}

\paragraph{Specification Step.}
Now, we apply Lemma~\ref{lem:waldstop} using the accumulation point $T_A$ as our initial point, the cycle end $X$ as our ending point, the constant function $Y_t = 1$ as our test function, and the draining-downcrossing points $\left(\dnb{i}\right)$ as our intervening points; we use $\bind$ to count the number of intervening points. To complete the proof, we must show that the following claims:
\begin{equation}\label{eq:tb_init}
    \ex{\dnb{1} - T_A} \leq \beta +  \frac{1}{\mu}\frac{F_1 \beta \sqrt{R}}{k - R} + \frac{1}{\mu}\frac{3}{2}\ln(\beta) + \frac{1}{\mu}\ln(F_1 D_1) ,
\end{equation}
\begin{equation}\label{eq:tb_cont}
    \ex{ \mintwo{X}{\dnb{i+1}} - \dnb{i} \middle | \bind \geq i} \leq \frac{D_2}{\mu \sqrt{R}} + \frac{D_3}{\mu R} + \frac{2}{\mu \tbthresh} 
\end{equation}
\begin{equation}\label{eq:tb_prob}
    \pr{ \bind \geq i+ 1\geq \bind \geq i} \leq \frac{1}{\tbthresh}.
\end{equation}


\paragraph{Completion of Proof assuming \eqref{eq:tb_init}, \eqref{eq:tb_cont}, and \eqref{eq:tb_prob}.}
Before proving the claims, we now prove the lemma. It suffices to give a bound on $\ex{X - \dnb{1}}$; applying Lemma~\ref{lem:waldstop} gives
\begin{align*}
    \ex{X- \dnb{1}} &\leq \tbthresh \left[ \frac{D_2}{\mu \sqrt{R}} + \frac{D_3}{\mu R} + \frac{2}{\mu \tbthresh}\right]\\
    &= \frac{2}{\mu} + \left[D_2 + \frac{D_3}{\sqrt{R}} \right]\max\left(\frac{1}{D_1 \sqrt{\mu \beta}}, \frac{1}{\sqrt{R}}\right). 
\end{align*}

\subsubsection{Proof of \eqref{eq:tb_init}.}
To bound $\ex{\dnb{1} - T_A}$, we make a coupling argument then apply basic results on M/M/1 busy periods. Moreover, instead of proving \eqref{eq:tb_init} directly, we first show a more general claim.
\begin{claim}\label{clm:tb_induct}
    For $\tbthresh \leq j \leq N(T_A) - R$, define $\eta_j$ as the first time after $T_A$ that $N(t) \leq R+ j$. Note that this means that $\eta_{N(T_A)} = T_A$ and $\eta_{\tbthresh} = \dnb{1}$. Then we have the following bound:
    \begin{equation*}
        \ex{\eta_{\tbthresh} - \eta_{j} \middle | \filt{\eta_j}} \leq \rem{R+j}(\eta_j) + \frac{1}{\mu}\sum_{i= \tbthresh}^{j}{\frac{1}{\mintwo{i}{k-R}}}. 
    \end{equation*}
\end{claim}
\newcommand{\remrj}{\rem{R+j}\left(\eta_j \right)}
Afterwards, we complete the proof by noting that $\left[N(T_A) - k\right]^+ \leq \left[N(T_A) - R \right]$, taking expectations, applying Jensen's inequality to the minimum function and the $\ln(\cdot)$ (which is concave), using the bound on $\ex{N(T_A) - R}$ from Claim~\ref{clm:taexpect}, then letting $h = \tbthresh$.


\paragraph{Proof of Claim~\ref{clm:tb_induct}.}
We prove Claim~\ref{clm:tb_induct} by induction. In the base case, suppose that $j = \tbthresh + 1$. Note that at time $\eta_{\tbthresh + 1}$, the numbers of jobs $N(\eta_{\tbthresh + 1} = R + \tbthresh + 1$ and the remaining time until the $(R+\tbthresh+1)$-th server turns on is $\rem{R + \tbthresh+1}\left(\eta_{\tbthresh + 1}\right)$. As such, we can simply wait until either that server turns on, in which case we can analyze the system as an M/M/1 busy period with departure rate $\mu \mintwo{R+\tbthresh+1}{k}$, or the number of jobs $N(t)$ drops below $R+\tbthresh + 1$ on its own. In other words, (using $j$ here to save space)
\begin{equation*}
    \ex{\eta_{j-1} - \eta_{j}\middle | \filt{\eta_{j}}} 
    \leq \remrj + 
    \frac{\ex{\left[N\left(\eta_j + \rem{R+j}\left(\eta_j\right)\right) - \left(R+(j-1)\right)  
        \right] \indc{\eta_{j-1} > \eta_{j} + \remrj} \middle | \filt{\eta_j}}}
    {\mu \mintwo{j}{k-R}}.
\end{equation*}
Now, we reframe the expectation as an expectation up to a stopping time. We note that, if $\eta_{j-1} > \eta_j + \remrj$, then we have that
\begin{equation*}
    N\left(\eta_j + \remrj \right) = N\left(\mintwo{\eta_j + \remrj}{\eta_{j-1}}\right).
\end{equation*}
Likewise, if $\eta_{j-1} \leq \eta_j + \remrj$, then
\begin{equation*}
     R + j - 1 =  N\left(\eta_{j-1}\right) = N\left( \mintwo{\eta_j + \remrj}{\eta_{j-1}}\right).
\end{equation*}
Using this and applying a simple coupling argument, one sees that
\begin{align*}
    &\ex{\left[N\left(\eta_j + \rem{R+j}\left(\eta_j\right)\right) - \left(R+(j-1)\right)  
        \right] \indc{\eta_{j-1} > \eta_{j} + \remrj} \middle | \filt{\eta_j}}\\
        &\;\; = \ex{N\left(\mintwo{\eta_j + \remrj}{\eta_{j-1}}\right) - (R + j - 1) \middle | \filt{\eta_j}}\\
        &\;\; \leq N\left(\eta_j\right) - (R + j - 1) = 1.
\end{align*}
Thus, we find that
\begin{equation*}
    \ex{\eta_{j-1} - \eta_{j}\middle | \filt{\eta_{j}}} 
    \leq \remrj + \frac{1}{\mu \mintwo{j}{k-R}}.
\end{equation*}

\paragraph{Inductive case.}
The inductive case proceeds in much the same way, except now, if $N(t)$ does drop below $R+j$ ``early'', then we can factor in the time that has elapsed in the value of $\rem{R+j}(\eta_j)$.
In particular, note that, since the $(R+j)$-th server would have already turned on,
\begin{equation*}
\ex{\eta_{\tbthresh} - \eta_j \middle |\filt{\eta_j}}\indc{\eta_j \geq \eta_{j+1} + \rem{R+j+1}(\eta_{j+1})}\leq \frac{1}{\mu}\sum_{i=\tbthresh}^{j}{\frac{1}{\mu \mintwo{i}{k-R}}}\indc{\eta_j \geq \eta_{j+1} + \rem{R+j+1}(j+1)}.
\end{equation*}
It follows that
\begin{equation*}
\ex{\eta_{\tbthresh} - \eta_j \middle |\filt{\eta_j}}\leq \rem{R+j}\left(\eta_j\right)\indc{\eta_j < \eta_{j+1} + \rem{R+j+1}\left(\eta_{j+1}\right)} + \frac{1}{\mu}\sum_{i=\tbthresh}^{j}{\frac{1}{\mu \mintwo{i}{k-R}}}.
\end{equation*}
Now, we note that
\begin{align*}
    \remrj \indc{\eta_j < \eta_{j+1} + \rem{R+1+j}\left(\eta_{j+1}\right)} &= \left[\remrj + \eta_j - \eta_j \right] \indc{\eta_j < \eta_{j+1} + \rem{R+1+j}\left(\eta_{j+1}\right)}\\
    &= \left[\rem{R+j}\left(\eta_{j+1}\right) + \eta_{j+1} - \eta_j \right] \indc{\eta_j < \eta_{j+1} + \rem{R+1+j}\left(\eta_{j+1}\right)}\\
   &\leq  \left[\rem{R+j+1}\left(\eta_{j+1}\right) + \eta_{j+1} - \eta_j \right] \indc{\eta_j < \eta_{j+1} + \rem{R+1+j}\left(\eta_{j+1}\right)}\\
   &= \left[\rem{R+j+1}\left(\eta_{j+1}\right) + \eta_{j+1} - \eta_j \right]^+,
\end{align*}
so that we find
\begin{equation*}
    \ex{\eta_{\tbthresh} - \eta_j \middle |\filt{\eta_j}}\leq \left[\rem{R+j+1}\left(\eta_{j+1}\right) + \eta_{j+1} - \eta_j \right]^+ + \frac{1}{\mu}\sum_{i=\tbthresh}^{j}{\frac{1}{\mu \mintwo{i}{k-R}}}.
\end{equation*}
Finally, we note that
\begin{equation*}
    \ex{\eta_{j} - \eta_{j+1} \middle | \filt{\eta_{j+1}}} \leq \ex{\mintwo{\eta_{j} - \eta_{j+1}}{\rem{R+j+1}\left(\eta_{j+1}\right)}\middle | \filt{\eta_{j+1}}} + \frac{1}{\mu \mintwo{j+1}{k-R}}.
\end{equation*}
Summing these final two expressions gives the inductive result, proving Claim~\ref{clm:tb_induct}. 

\paragraph{Using Claim~\ref{clm:tb_induct}.}
Thus, we obtain that, using $H_i$ to denote the $i$-th harmonic number,
\begin{align*}
    \ex{\dnb{1} - T_A\middle | \filt{T_A}} &\leq \beta + \frac{1}{\mu}\frac{\left[N(T_A) - k\right]^+}{k-R} + \frac{1}{\mu}\left[H_{\mintwo{N(T_A)-R}{k-R}} - H_{\tbthresh}\right]\\
    &\leq \beta + \frac{1}{\mu}\frac{\left[N(T_A) - R\right]^+}{k-R} + \frac{1}{\mu}\ln\left(\frac{\mintwo{N(T_A) - R}{k-R}}{M_L}\right). 
\end{align*}
Taking expectations and applying Jensen's inequality twice, we find
\begin{align*}
     \ex{\dnb{1} - T_A\middle | \filt{T_A}} &\leq \beta + \frac{1}{\mu} \frac{F_1 \mu \beta \sqrt{R}}{k-R} + \frac{1}{\mu}\ln\left(\frac{F_1 \mu \beta \sqrt{R}}{M_L}\right)\\
     &\leq \beta + \frac{1}{\mu} \frac{F_1 \mu \beta \sqrt{R}}{k-R} + \frac{1}{\mu}\ln\left(\frac{\min\left(F_1 \mu \beta \sqrt{R}, k - R\right)}{\min\left(\max\left(1,\frac{\sqrt{R}}{D_1 \sqrt{\beta}}\right) , k-R\right)}\right)\\
     &\leq \beta + \frac{1}{\mu} \frac{F_1 \mu \beta \sqrt{R}}{k-R} + \frac{1}{\mu}\ln\left(F_1 D_1 \beta^{3/2}\right)\\
     &= \beta + \frac{1}{\mu} \frac{F_1 \mu \beta \sqrt{R}}{k-R} + \frac{1}{\mu}\frac{3}{2}\ln\left(\beta\right) + \frac{1}{\mu} \ln\left(F_1 D_1\right). \hfill \Halmos
\end{align*}

\subsubsection{Proof of \eqref{eq:tb_cont}.}\label{sec:downtodown}
To bound the expectation $\ex{\mintwo{\dnb{i+1}}{X} - \dnb{i} \middle | \filt{\dnb{i}}}$, we split the interval into two parts, $\left[\mintwo{\unb{i}}{X} - \dnb{i}\right]$ and $\left[\dnb{i+1} - \dnb{i}\right]$.


To bound the expectation of the first quantity, it suffices to note that, if we couple the system to an M/M/$\infty$, the coupled number of jobs $\ncouple(t)$ will reach $R + \tbthresh$ only after the original system. Using Claim~\ref{clm:mminf_up} to bound this passage time, we thus know that
\begin{align*}
    \ex{\mintwo{\unb{i}}{X} - \dnb{i}\middle | \filt{\dnb{i}}} &\leq \ex{\mintwo{T^{M/M/\infty}_{(R+\tbthresh - 1)\to (R+ \tbthresh)} + \dnb{i}}{X} - \dnb{i} \middle | \filt{\dnb{i}}}\\
    &\leq \ex{T^{M/M/\infty}_{(R+\tbthresh - 1)\to (R+ \tbthresh)}}\\
    &\leq \frac{D_2}{\sqrt{R}}.
\end{align*}

To bound the expectation of the second quantity, we provide two bounds. First, we again make use of the ``wait-busy'' idea; as we argued in the proof of \eqref{eq:tb_init},
\begin{equation*}
    \ex{\dnb{i+1} - \unb{i}\middle | \filt{\unb{i}}} \leq \ex{\mintwo{\dnb{i+1} - \unb{i}}{\beta}\middle | \filt{\unb{i}}} + \frac{1}{\mu \tbthresh}.
\end{equation*}
From here, we note, by coupling to an M/M/1 with arrival rate and departure rate both equal to $k \lambda$, we can bound $\ex{\mintwo{\dnb{i+1} - \unb{i}}{\beta}\middle | \unb{i} < X}$ by the expected minimum between $\beta$ and the length of a single-job busy period in that system. Applying Claim~\ref{clm:contint}, we can complete the proof, finding that
\begin{equation*}
    \ex{\mintwo{\dnb{i+1} - \unb{i}}{\beta}\middle | \filt{\unb{i}}} \leq D_1 \frac{\sqrt{\beta}}{\sqrt{\mu R}} + \frac{6}{\mu R}.
\end{equation*}

For the second bound, we simply note that, during the draining phase, the number of busy servers $Z(t) \geq R+1$. It follows from a simple coupling argument that
\begin{equation*}
     \ex{\mintwo{\dnb{i+1} - \unb{i}}{\beta}\middle | \filt{\unb{i}}} \leq \frac{1}{\mu}.
\end{equation*}
Combining the bounds pessimistically, we find that
\begin{align*}
    \ex{\mintwo{\dnb{i+1}}{X} - \dnb{i} \middle | \filt{\dnb{i}}} &\leq \frac{D_2}{\mu \sqrt{R}} + \frac{D_3}{\mu R} + \frac{1}{\mu\tbthresh} + \min \left(D_1 \frac{\sqrt{\beta}}{\sqrt{\mu R}}, \frac{1}{\mu}\right)\\
    &\leq  \frac{D_2}{\mu \sqrt{R}} + \frac{D_3}{\mu R} + \frac{2}{\mu \tbthresh} 
\end{align*}


\subsubsection{Proof of \eqref{eq:tb_prob}.}
To bound the probability of an additional downcrossing, we again make a coupling argument. In particular, we couple again to the system which only has $R$ servers busy, which gives an upper bound on the number of jobs in the system $N(t)$. If, in our coupled system, we reach $\ncouple(t) = R + \tbthresh$ before we reach $\ncouple(t) = R$, then another upcrossing \emph{must} have previously occurred in the original system, and thus another downcrossing must also occur. But, of course, we know classically that the probability that this happens is just $\frac{1}{\tbthresh}$; this is precisely what is asserted by \eqref{eq:tb_prob}. \hfill \Halmos

==> theorem2/theorem2.tex <==
\newcommand{\erbterm}{e^{\frac{1}{24 R \setuptime}}}
\newcommand{\qcouple}{\Tilde{Q}}
\newcommand{\tlba}{\tau_L + \beta}
\newcommand{\mtb}{\mintwo{\tau_i + \beta}{\tau_{i+1}}}
\newcommand{\upc}{\gamma}
\newcommand{\dnc}{\alpha}
\newcommand{\ncac}{\ncouple}
\newcommand{\cind}{n_\alpha}
\newcommand{\tac}{\Tilde{T}_A}

We now show how to apply the techniques from this paper to obtain an improvement of the main theorem of \cite{WHW}.

\improvement*

\paragraph{Improvement.} This theorem is an improvement both practically and theoretically. As shown in Figure~\ref{fig:appxA}, the lower bound of Theorem~\ref{thm:improvement} is much closer to what we observe in the data than the lower bound shown in \cite{WHW}. Furthermore, in \cite{WHW}, the lower bound on the mean number of jobs in queue $\ex{Q(\infty)}$ included a $\log(k)$ in the denominator; as one scaled the system size, this term would, paradoxically, drive their lower bound to $0$. In Theorem~\ref{thm:improvement}, no such diverging term exists; in fact, we show in Section~\ref{sec:tightness} that it matches our upper bound up to multiplicative constants.

\paragraph{Proof Outline.}
We prove Theorem~\ref{thm:improvement} in much the same way that we proved Theorem~\ref{thm:main} (via the method discussed in Section~\ref{sec:keyideas}). We apply the Renewal-Reward Theorem to the number of jobs in the queue $Q(t)$ using the same renewal cycle, and have a lemma which bounds the numerator and two lemmas which together bound the denominator. The pair of lemmas focus on bounding $\ex{T_A}$ and $\ex{X - T_A}$, respectively, where one should recall that the stopping time $T_A \triangleq \minpar{t >0: Z(t) \geq R+1}$ is the first moment during a renewal cycle that the $(R+1)$-th server is on. In particular, we show the following lemmas.
\begin{restatable}[Lower bound on Cycle Integral]{lemma}{lbint}\label{lem:lb_int}
    Let $\ibp{x}{i}$ is the expected time integral of the number of jobs in system for an M/M/1 with arrival rate $k \lambda$ and departure rate $\mu(R + i)$, started with $x$ jobs in the system. For the time integral of a the number of jobs in queue $Q(t)$ over a renewal cycle, we have the bound:
    \begin{equation*}
        \ex{\int_0^{X}{Q(t) \dd t}} \geq L_1 \beta^2 \sqrt{R} + \ibp{\left[L_1 \beta \sqrt{R} - (k-R) \right]^+}{k - R}.
    \end{equation*}
\end{restatable}
\begin{restatable}[Upper bound on Accumulation Phase Length]{lemma}{ubacc_cycle}\label{lem:ubacc_cycle}
    Recall that $T_A \triangleq \minpar{t > 0: Z(t) \geq R + 1}$.Then
    \begin{equation*}
        \ex{T_A} \leq \erbterm \left( \sqrt{1 + \frac{1}{2 R \setuptime} } \right) 
         \left[ 
            1 
            + \frac{e^{\frac{1}{12 R}}}{\sqrt{2 \mu \beta}}       
        \right] \beta \leq 2.16 * \beta.
    \end{equation*}
\end{restatable}
\begin{restatable}[Upper bound on Draining Phase Length]{lemma}{ubdr_cycle}\label{lem:ubdr_cycle}
    Let $\bp{x}{i}$ is the expected length of an M/M/1 busy period with arrival rate $k \lambda$, departure rate $\mu(R + i)$, started with $x$ jobs in the system. Then, one can bound $\ex{X-T_A}$ by
    \begin{equation*}
        \ex{X-T_A} \leq \beta +  \frac{1}{\mu}\frac{F_1 \beta \sqrt{R}}{k - R} + \frac{1}{\mu}\frac{3}{2}\ln(\beta) + \frac{1}{\mu}\ln(F_1 D_1)
        +
        \frac{2}{\mu} 
        + \left[D_2 + \frac{D_3}{\sqrt{R}} \right]\max\left(\frac{1}{D_1 \sqrt{\mu \beta}}, \frac{1}{\sqrt{R}}\right),
    \end{equation*}
    where $F_1$, $D_1$, $D_2$, and $D_3$ are constants not depending on system parameters. 
\end{restatable}

We prove each of these lemmas in sequence.


\subsection{Proof of Lemma~\ref{lem:lb_int}.}\label{sec:LBint}
\input{theorem2/lemma_LB_int}


\subsection{Proof of Lemma~\ref{lem:ubacc_cycle}.}\label{sec:ubacc_cycle}

\input{theorem2/lemma_UB_TA}

\subsection{Proof of Lemma~\ref{lem:ubdr_cycle}.}\label{sec:ubdr_cycle}

\input{theorem2/lemma_UB_TB}






